Self-Supervised Category-Level Articulated Object Pose Estimation with Part-Level SE(3) Equivariance

Category-level articulated object pose estimation aims to estimate a hierarchy of articulation-aware object poses of an unseen articulated object from a known category. To reduce the heavy annotations needed for supervised learning methods, we present a novel self-supervised strategy that solves this problem without any human labels. Our key idea is to factorize canonical shapes and articulated object poses from input articulated shapes through part-level equivariant shape analysis. Specifically, we first introduce the concept of part-level SE(3) equivariance and devise a network to learn features of such property. Then, through a carefully designed fine-grained pose-shape disentanglement strategy, we expect that canonical spaces to support pose estimation could be induced automatically. Thus, we could further predict articulated object poses as per-part rigid transformations describing how parts transform from their canonical part spaces to the camera space. Extensive experiments demonstrate the effectiveness of our method on both complete and partial point clouds from synthetic and real articulated object datasets.

==> articles/method_old.tex <==
% !TEX root = ../main.tex

\section{Method}

% outline for the proposed method
% \begin{itemize}
%     \item Part proposal module.
%     \item Part motion prediction strategy.
%     \begin{itemize}
%         \item Joint modeling strategy (point-based strategy \& assumptions and limitations)
%     \end{itemize}
%     \item Part-level equivariance. 
%     \begin{itemize}
%         \item Method.
%         \item Motivation.
%     \end{itemize}
% \end{itemize}

\begin{figure*}[ht]
    \centering
    %   \includegraphics[width=1.0\textwidth]{./imgs/overview-33.pdf}
      \includegraphics[width=1.0\textwidth]{./imgs/abs-overview.pdf}
      \vspace{-10pt}
    \caption{
      \footnotesize
    %   \textcolor{}{}
    % \textcolor{myblue}{
      Overview of the proposed self-supervised articulated object pose estimation strategy.
    %   }
    %   part articulated pose estimation strategy. 
    The method takes a complete or partial point cloud of an articulated object as input, factorizes canonical shapes, object structure, and the articulated object pose from it. 
    The network is trained by a shape reconstruction task. 
    Part-level SE(3) equivariant features are learned  by iterating between part pose estimation and pose-aware equivariant point convolution. 
    % reconstructs canonical shapes 
    % at different levels 
    % and predicts part rigid transformations across shapes in those canonical spaces and the camera space for articulated object pose estimation. 
    % reconstructs a set of invariant reference frame $ \{ Z_i \}$ for each part $i$,  and estimates three-levels of part poses to transform each part to the camera space for shape reconstruction. 
    % The articulated object pose estimation network is trained via a shape reconstruction-based self-supervised loss. 
    % The network is trained via a shape reconstruction-based self-supervised task. 
    %   The method takes a complete or partial point cloud $X$ of an articulated object as input,
    %   reconstructs a set of invariant reference frame $ \{ Z_i \}$ for each part $i$, 
    % %   in its canonical part space with part pose canonicalized, 
    %   reconstructs an invariant shape $Z$ in the canonical object space 
    % %   for the whole shape with object orientation, joint parameters, and part articulation state normalized, 
    %   and estimates three-levels of part 
    % %   reconstructs an invariant reference frame $Z = \{ Z_i \}$ with all part poses canonicalized and estiamtes 
    %   part articulated poses $\{ P_i \}$ to transform each part from its reference frame to  the observed shape for shape reconstruction-based self-supervision.
    %   shape in the reference frame to the shape in the observed camera space for reconstruction based self-supervision.
    %   ``Invariant Properties'' include the part-by-part canonical shape reconstruction $\{ Z_i \vert 1\le i\le K\}$, and the predicted pivot point $\mathbf{p}_{i,j}^v$ for each two adjacent part $(i,j)\in \mathcal{E}_{\mathcal{T}}$ in the predicted kinematic chain. 
    %   ``Per-part Per-rot Pose-related Parameters'' denote predicted parameters for part rigid transformation for each $g_j\in G_g$. 
     % Please refer to Section~\ref{sec_method_ssl_method} for details.
    %   of such predicted invariant/equivariant properties. 
    %   The module ``Invariant Properties Prediction'' predicts per-part canonical shape $\{ Z_i \}$, per-part central point $\{ \mathbf{p}_i^c \}$, and per-part pair pivot point $\{ \mathbf{p}_{i,j}^v \}$ taking per-part equivariant feature as input. 
    %   The module ``Invariant Properties Prediction'' predicts per-part per-rot parameters for further part rigid transformation calculation, including like axis $\{ \mathbf{u}_i^j \}$, rotation angles $\{ \theta_i^j \}$, and translation scalars $\{ s_i^j \}$. 
    %   Please refer to Section~\ref{sec_method_ssl_method} for details of such two modules.
      \textcolor{mygreen}{Green} lines (\textcolor{mygreen}{$\leftarrow$}) denote procedures for feeding the estimated part poses back to the  pose-aware point convolution module.
    %   feeding back the estimated part poses to the feature backbone to participate in the pose-aware point convolution. 
    %   (the design of iterative pose estimation). 
%  inter-part feature communication process.
    %   to perform iterative part pose estimation.
    %   Overview of the proposed self-supervised 6D part pose estimation strategy. 
    %   Taking a complate or depth point cloud $X$ of an articulated object as input, our method reconstructs an invariant reference frame $Z = \{Z_i\}$ with all part poses canonicalized and estiamtes the 6D part poses $\{ P_i \}$ that can transform the shape in the reference frame to the shape in the observed camera space. 
    %   The self-supervision is added from a shape reconstruction task. 
    %   Together with the inter-part equivariant feautre communication design, the estiamted part pose could be fed back to the backbone for better equivariant feature extraction. 
    %   \textcolor{gray}{Gray} lines (\textcolor{gray}{$\rightarrow$}) here are common pipelines for both shapes containing revolute parts or prismatic parts, while \textcolor{myblue}{blue} lines (\textcolor{myblue}{$\rightarrow$})  are designed to process revolute parts only.  \textcolor{mygreen}{Green} lines (\textcolor{mygreen}{$\rightarrow$}) denote procedures for feeding back the estimated part poses for better point equivariant features.      
    %   Taking complete or depth point clouds of an articulated object as input, our 
    %   the EPN-based backbone is applied to extract per-point per-rot feature vectors $\{\mathbf{f}({x}_i, \mathbf{g}_j) \vert x_i\in X, g_j\in G_g\}$. 
    %   The proposed method takes complete or depth point clouds as input, 
    % Overview of the proposed method. 
    % Loss functions written here is for complete point clouds. The method could be applied on partial point clouds by changing the bidirectional chamfer distance function $\text{CD}(\cdot, \cdot)$ in the loss function to unidirection chamfer distance function $\text{UniCD}(\cdot, \cdot)$, as discussed in section~\ref{sec_method_ssl_method}. $\mathcal{L}_{reg}$ here denotes losses added for joint-related constraints. $\lambda$ is the hyperparameter added for the loss function. 
    }
    \label{fig_overall_pipeline}
    % \vspace{-5pt}
    \vspace{-10pt}
\end{figure*}

% Our key contribution is to present a self-supervised framework achieving part shape, part structure, joint, and part pose disentanglement. We achieve this leveraging part-level SE(3) equivariance from a novel equivariant network design.

% \zz{Not necessary to use a separate section for Overview?}
In this section, we present our method for self-supervised category-level articulated object pose estimation. 
% To estimate category-level pose for articulated objects, we need to factorize part-related pose and shape information at a finer level than for rigid objects. 
% The key to solving the problem is letting the network propose canonical shapes as the reference frame to define articulated object pose during the self-supervised training so that articulated object pose could be estimated by predicting rigid transformations that bridge part shapes in different spaces. 
% Our method lets the network predict the category-level canonical object shape, canonical part shapes, object structure, and the articulated object pose from input shapes. 
% Our method lets the network learn category-level canonical object space, a set of canonical part spaces, and articulated object poses from a set of articulated objects. 
% category-level canonical spaces for both parts and the object as their reference frames, predict the structure of the object, and the articulated object pose from 
% input shapes
% The key to solving this task in a self-supervised way 
% % without any pose annotations, part segmentations, or even canonical frames for pose definition 
% is letting the network propose canonical spaces as reference frames for parts and the object, and predict articulation-aware rigid transformations across those spaces. 
% The key to solving the problem is letting the network propose canonical shapes as reference frames and predict articulation-aware rigid transformations across those spaces. 
% It requires the network to have the concept of parts and disentangle part-level properties from the input articulated object.
% infer part-level properties from the input articulated object. 
% Inferring such information requires the network to factorize pose and shape-related information at the part level. 
% To solve this problem in a self-supervised manner, we wish to achieve part-level SE(3)-equivariance at the feature level (sec.~\ref{sec_method_revisit}) so that such features are more friendly for part-level pose and shape disentanglement. 
% Inferring part poses requires us to factorize information at the part level.
% the network to factorize information at the part level.
% information to be factorized at the part level. 
% Therefore, we wish to acquire part-level SE(3) equivariant features to reduce the difficulty of the disentanglement problem, considering the part-level SE(3) equivariant property of part poses.
% We first propose a part-level SE(3) equivariant network to learn part-level SE(3) equivariant features
We first propose to learn part-level SE(3) equivariant features through a novel pose-aware equivariant point convolution module to reduce the difficulty of the decomposition problem (sec.~\ref{sec_method_revisit}). 
Based on such features, we then design a disentanglement strategy that factorizes invariant canonical shapes, 
% canonical spaces, 
object structure, and articulated object poses from input shapes (sec.~\ref{sec_method_ssl_method}). 
We hope that the category-level canonical object space and part spaces could be induced automatically from input shapes taking advantage of part-level SE(3) equivariance. 
% so that the decomposition problem could be made network-friendly. 
% To reduce the difficulty of the highly ill-posed disentanglement problem, we wish to acquire part-level SE(3) equivariant features (sec.~\ref{sec_method_revisit}) so that we can factorize invariant canonical spaces, object structure, and articulated object poses from the input shapes (sec.~\ref{sec_method_ssl_method}). 
%the problem is solvable in a self-supervised setting.%, considering the part-level SE(3) equivariant property of part poses.
% Based on the part-level SE(3) equivariant property of part poses, we wish to acquire such property in the feature level to reduce the difficulty of the tough disentanglement problem.
% Inspired by the contribution of SE(3)-equivariant features to self-supervised pose estimation for rigid objects~\cite{li2021leveraging}, we wish to acquire part-level SE(3)-equivariance to make the problem more friendly to solve in a self-supervised way. 
% Therefore, to make the problem more friendly to solve in a self-supervised way, we wish to seek part-level SE(3)-equivariance 
% from 
% features considering the contribution of SE(3)-equivariance features to the self-supervised pose estimation for rigid objects~\cite{li2021leveraging} (sec.~\ref{sec_method_revisit}). 
% With such part-level equivariant features, we design a part shape, object structure, and part disentanglement strategy to factorize useful part-level information from input articulated objects (sec.~\ref{sec_method_ssl_method}). 
% Then, with such equivariant features, 
%With such equivariant features, 
% with the part-level equivariant features, 
%we design a disentanglement strategy 
% for articulated pose estimation 
%that factorizes invariant canonical spaces, object structure 
% such as part adjacency relationship and the kinematic chain 
%, and 
% part-level equivariant 
% articulation-aware part poses
%articulated object poses
% -related equivariant information 
%from the input articulated object
% at both part-level and object-level, 
% including canonical part shapes, object structure, and articulated object pose 
Further, we adopt a part-by-part shape reconstruction task that combines the factorized information for 
% input 
shape reconstruction to self-supervise the factorization (sec.~\ref{sec_method_self_supervised_task}). 
Our method assumes a category-level setting where input shapes have the same kinematic chain. 
For notations frequently used in the following text, $N$, $C$ and $K$ denote the number of points, feature dimension, and the number of parts of the input shape respectively. 
% We use $T$ to represent a rigid transformation. 
% 
% In the following text, 
% we use $N$ to denote the number of points in the input shape, while $K$ for the number of parts. 
% we use $N$ and $K$ to denote the number of points and parts in the input shape respectively

%%%% %%%%%
% \summary{Overview}
% In this section, we present our self-supervised framework that performs part shape, object structure, and articulated pose disentanglement from an articulated object leveraging part-level SE(3)-equivariance.
% % disentangles part shape, part structure, part joint, and part pose from an articulated object leveraging part-level SE(3)-equivariance. 
% % \todo{for the following sections?}

% \summary{Contents}\zz{Necessary?}
% We first introduce the equivariant network design to achieve part-level SE(3)-equivariance in section~\ref{sec_method_revisit}.
% % Based on such part-level SE(3)-equivariant features, we further introduce the designed strategy to conduct the shape, structure, and pose disentanglement for articulated objects 
% % to achieve the shape, structure, and pose disentanglement for articulated object pose estimation 
% % (sec.~\ref{sec_method_ssl_method}), and further the shape reconstruction-based self-supervised task to guide the network's learning (~\ref{sec_method_self_supervised_task}). 
% In the following text, we first introduce our design to achieve part-level SE(3)-equivariance in section~\ref{sec_method_revisit}, then the shape, structure, pose disentanglement strategy in section~\ref{sec_method_ssl_method}, and further the part-by-part shape reconstruction task for self-supervision in section~\ref{sec_method_self_supervised_task}. 
%%%% %%%%%


% section~\ref{sec_method_ssl_method},~\ref{sec_method_self_supervised_task}. 
% of those four part-level properties in section~\ref{sec_method_ssl_method},~\ref{sec_method_self_supervised_task}. 

% To achieve part-level SE(3)-equivariance, we 
% reconstruct 
% % an invariant canonical 
% a category-level reference frame $Z_i\in \mathbb{R}^{N_i^z\times 3}$ for each part $1\le i\le K$; 
% 2) predict part association and part kinematics related parameters like kinematic chain, and joint-related parameters; 
% 3) estimate part pose $P_i\in (\mathbf{R}^i, \mathbf{t}^i)$ for each part $i$ from its reference frame $Z_i$ to the observed shape $X$. 
% % $Z\in \mathbb{R}^{N_z \times 3}$ for $X$ with all parts' pose canonicalized; 2) estimate part pose $P^i = (\mathbf{R}^i, \mathbf{t}^i)$ for each part $i$ from $Z$ to the observed shape $X$. 
% % and the prior knowledge of the number of parts $K$ for all shapes in the category, our method aims to 
% % 1) Reconstruct a category-level reference frame $Z\in \mathbb{R}^{N_z \times 3}$ for $X$ with all parts' pose canonicalized; 
% % 2) Estimate the pose $P^i = (\mathbf{R}^i, \mathbf{t}^i)$ for each part $i$ from $Z$ to the observed shape $X$. 
% Since we target at part-level understanding for the input object, the network should also decompose the input shape into different parts based on part rigid transformations.
% % To perform this task, the network should also 
% % decompose the input shape into different parts based on part rigid transformation.
% % also naturally decompose the input shape into different parts based on part rigid transformation. 

% \todo{move such definitions to intro}
% Part-level invariant canonical shape reconstruction requires the reconstruction to be not only invariant to its own rigid transformation, but also invariant to other parts'.
% % the pose change of itself, but also invariant to pose changes of other parts.
% If we do not assume the kinematic constraints between different parts, this suggests that the canonical part shape reconstruction should be invariant to the cartesian product of $K$ SE(3) groups, 
% % i.e., $Z_i(\{ X_j \vert 1\le j \le K \}) = Z_i(\{ T_{A_j}(X_j) \vert A_j\in G_A, 1\le j\le K \}), \forall 1\le i\le K$. 
% i.e., $Z_i(T_{(A_j)_{1\le j\le K}}[X]) = Z_i(X)$.

% Part-level equivariant pose estimation indicates the estimated part pose for part $i$ to change by the same transformation $A_i$ applied on part $i$ of the input point cloud, i.e. $P_i((T_{A_i})(X)) = T_{A_i}[P_i(X)]$. 
% % For equivariant part pose estimation, we want the estimated pose for part $i$ to change by the same transformation ${A_i}$ applied to the part $i$ of the input point cloud, e.g. $P_i((T_{A_i})(X)) = T_{A_i}[P_i(X)]$. 
% For articulated objects, we also want the estimated pose for part $i$ invariant to the pose change of other parts, i.e. 
% % to be invariant to other parts' pose change, e.g. 
% $P_i((T_{A_j})_{1\le j\neq i\le K}[X]) = P_i(X)$. 
% Combining such two conditions, we can arrive at the condition that equivariant part pose estimation should satisfy: 
% % $P_i((T_{A_j})_{1\le j\le K}[X]) = T_{A_i}[P_i(X)]$.
% $P_i(T_{(A_j)_{1\le j\le K}}[X]) = T_{A_i}[P_i(X)]$.


%%%%%%% v11 %%%%%%%%
% Invariant canonical shape reconstruction for articulated objects suggest the reconstruction should be invariant to all parts' rigid transformation. 
% Thus, we propose to reconstruct each part in the canonical space $\{ Z_i \vert 1\le i\le K \}$ and further assemble them together for the canonical reconstruction of the whole shape. 
% % To estimate category-level part pose, we wish that the network should reconstruct 
% % Invariant canonical shape reconstruction for articulated objects suggest that the reconstruction should be invariant to all parts' rigid trnasformations.
% % Thus, to reconstruct an invariant canonical point cloud $Z$, we propose to reconstruct each part in the canonical space $\{Z_i\}_{1\le i\le K}$ and further assemble them together for the canonical reconstruction of the whole shape.
% % Furthermore, to estimate the category-level 6D part pose, we wish that the network should reconstruct part shapes in a category-level canonical reference frame.
% % Then, the whole shape is also reconstructed in a category-level canonical space. 
% Canonical part reconstruction requires the reconstruction to be not only invariant to the pose change of itself, but also invariant to pose changes of other parts.
% If we do not assume the kinematic constraints between different parts, this suggests that the canonical part shape reconstruction should be invariant to the cartesian product of $K$ SE(3) groups, i.e., $Z_i(\{ X_j \vert 1\le j \le K \}) = Z_i(\{ T_{A_j}(X_j) \vert A_j\in G_A, 1\le j\le K \}), \forall 1\le i\le K$, termed as ``part-level'' invariance. 

% Equivariant part pose estimation indicates the estimated part pose for part $i$ to change by the same transformation $A_i$ applied on part $i$ of the input point cloud, i.e. $P_i((T_{A_i})(X)) = T_{A_i}[P_i(X)]$. 
% % For equivariant part pose estimation, we want the estimated pose for part $i$ to change by the same transformation ${A_i}$ applied to the part $i$ of the input point cloud, e.g. $P_i((T_{A_i})(X)) = T_{A_i}[P_i(X)]$. 
% For articulated objects, we also want the estimated pose for part $i$ invariant to the pose change of other parts, i.e. 
% % to be invariant to other parts' pose change, e.g. 
% $P_i((T_{A_j})_{1\le j\neq i\le K}[X]) = P_i(X)$. 
% Combining such two conditions, we can arrive at the condition that equivariant part pose estimation should satisfy: $P_i((T_{A_j})_{1\le j\le K}[X]) = T_{A_i}[P_i(X)]$.
% Similarly, we call such property ``part-level'' equivariance.
%%%%%%% v11 %%%%%%%%

% Recently, there is a work demonstrating the effectiveness of using SE(3)-equivariant network to tackle the self-supervised pose estimation problem for rigid objects by properly extracting invariant and equivariant properties from the equivariant feature and using a shape reconstruction task to self-supervise the network's learning~\cite{li2021leveraging}.

% The main idea is that object pose is an equivariant property that would change equivalently to the rigid transformation of the input object.
% To leverage the property of equivariant features for part pose estimation, we propose to use SE(3)-equivariant network as our feature backbone. 
% We also add a pose-aware inter-part equivariant feature communication design for part-level equivariant features (sec.~\ref{sec_method_revisit}). 
% % with the design of pose-aware inter-part equivariant feature communication strategy for better part-level equivariant features (sec.~\ref{sec_method_revisit}). 
% Then, we design a motion-based part-by-part shape reconstruction strategy by letting the network reconstruct an invariant reference frame for each part, and use the estimated part poses to transform them to the camera space for shape reconstruction-based self-supervision (sec.~\ref{sec_method_ssl_method},~\ref{sec_method_self_supervised_task}).
% transform parts to the canonical object space, predict the kinematic chain and other part kinematics-related parameters, and further estimate 6D part pose based on kinematic constraints to transform reconstructed shapes to the camera space for shape reconstruction (sec.~\ref{sec_method_ssl_method},~\ref{sec_method_self_supervised_task}).
% predict part kinematics-related properties  to assemble parts together, and further estimate 6D part poses to transform constructed parts for shape reconstruction (sec.~\ref{sec_method_ssl_method},~\ref{sec_method_self_supervised_task}).

% Here in our method, we also want to leverage the property of equivariant features for part pose estimation. 
% Furthermore, we wish for part-level equivariant features that can better support the above invariant/equivariant part-level properties prediction. 
% To seek for such features, we propose
% % Thus, we propose 
% a pose-aware inter-part equivariant feature communication strategy to disentangle the pose change of other parts from the current part's equivariant feature learning. 


% In the following text, we first revisit the design of EPN~\cite{chen2021equivariant} and our further design for better part-level equivariant features in section~\ref{sec_method_revisit}. 
% Then the proposed self-supervised shape reconstruction-based part pose estimation task is elaborated in section~\ref{sec_method_ssl_method}. 
% At last, loss function for self-supervision and reguralization is stated in section~\ref{sec_method_self_supervised_task}. 
% to disentangle other parts' pose change from the part own equivariant feature learning. 
% It requires per-point pose as additional inputs to perform feature convolution, which suggests an iterative pose estimation procedure. 

%%% move to section 3.1 %%%
% Therefore, our feature backbone takes the input point cloud $X$ and estimated per-point pose $P$ (optional) as input to extract per-point per-rotation feature: ${F}\in \mathbb{R}^{n\times C\times \vert G_g \vert} = \phi(X) = \{ \mathbf{f}(\mathbf{x}_i, g_j) \}$, where $\vert \{ \mathbf{x}_i \} \vert = n$, and $g_j\in G_g$. 
% % \todo{per-point equivariant feature...}
% We ommit the estimated pose-related input to the feature backbone in the notation and simply use $\phi(X)$ in the following text.
%%% move to section 3.1 %%%
% % First, section~\ref{sec_method_notations} aims to give a brief explanation on used notations. 
% % In section~\ref{sec_method_notations}, we first list some notations used here. 
% As a background, we first briefly revisit 
% % As a background, in section~\ref{sec_method_revisit}, we briefly revisit 
% Equivariant Point Network~\cite{chen2021equivariant} 
% % based on which we design our feature backbone for input point clouds 
% , the way it benefits self-supervised pose estimation for rigid objects~\cite{li2021leveraging}, and further some special designs j

% in section~\ref{sec_method_revisit}.
% % how it can be used in self-supervised pose estimation for rigid objects~\cite{li2021leveraging}. 
% After that, the proposed self-supervised 6D part pose estimation strategy is elaborated in section~\ref{sec_method_ssl_method}.
% Then in the following sections, we highlight two designs for part pose estimation, namely joint prediction strategy (sec.~\ref{sec_method_joint_prediction}) and part pose-aware inter-part equivariant feature communication strategy (sec.~\ref{sec_method_inv_feat_communication}).
% At last, some implementation details are stated in section~\ref{sec_imple_details}.
% while details of two components of the method are presented in the following two sections, namely joint prediction (sec.~\ref{sec_method_joint_prediction}) and the design of pose-aware inter-part invariant feature communication (sec.~\ref{sec_method_inv_feat_communication}).
% In section~\ref{sec_method_ssl_method}, we introduce the proposed self-supervised part 6D pose estimation strategy.
% In section~\ref{sec_method_joint_prediction}, we explain our joint prediction strategy for part pose calculation.
% At last, in section~\ref{sec_method_inv_feat_communication}, we introduce the pose-aware inter-part invariant feature communication strategy for better equivariant part features and further part-level properties.

% \subsection{Notations} \label{sec_method_notations}
% For point clouds, the input observed shape is denoted as $X$. The reconstructed shape for the rotation element $g_j\in G_g$ is denoted as $Y^j$. Part shapes are denoted as $\{X_i\}_{1\le i\le K}$, where $i$ is the index of the part.  
% For features, we use capital letters to represent shape equivariant feature output by the equivariant network backbone: $F\in \mathbb{R}^{N\times C\times \vert G_g\vert}$, while the bold letters to denote the SE(3)-invariant feature obtained by transforming the equivariant feature through pooling along the rotation group dimension $\vert G_g\vert$. 
% A shape is represented by a hollow capital letter: $\mathbb{S}$ denotes the input ground-truth shape, $\mathbb{S}_{i}$ denotes the $i$-th part in the input shape, $\hat{\mathbb{S}}_i$ denotes the reconstructed $i$-th part and $\hat{\mathbb{S}}$ represents the reconstructed whole shape. 
% Since we use point clouds for part shape representation, sometimes we need to represent shapes via point coordinate matrices for convenient part transformation representation. 
% Thus, $\mathbf{P}$ denotes the coordinate matrix of the input whole shape, $\mathbf{P}_i$ represents the coordinate matrix of the part $i$. Thus, $\hat{\mathbf{P}}$ represents the coordinate matrix of the reconstructed shape, $\hat{\mathbf{P}}_i$ is that of the reconstructed part $i$.
% % Matrices for reconstructed shapes can be obtained by adding hats on those ground-truth matrices. 
% % todo: add notations for shape canoniical space / part canonical space / and so on...
% Moreover, to decompose part poses from part shapes given an observed shape, we treat the whole shape generation process as a part-by-part assembly process transforming between different spaces via rigid transformation. 
% Thus, we define different kinds of shape spaces, namely part canonical space (PC), shape canonical space (SC), and observed camera space. Part shapes and coordiante matrices are denoted by adding upper food marks to their corresponding notations, such as $\hat{\mathbb{S}}_i^{PC}$. 

% The joint between two parts $\mathbb{S}_{i}$ and $\mathbb{S}_j$ is represented by the joint direction $\mathbf{u}_{i,j}$ and the pivot point $\mathbf{q}_{i,j}$. 
% For part rigid transformation related parameters, the rotation matrix for the part $i$ is represented by the black capital latter $\mathbf{R}_i$, and the translation vector for the part is denoted as $\mathbf{t}_i$. 
% % Rotation matrix and translation vector for the rigid transformation from part canonical space to shape canonical space are denoted as $\mathbf{R}_i^{C}$ and $\mathbf{t}_i^{C}$, respectively. 
% We assume that all shapes in one category have a same number of parts and use $K$ to denote the predefined part number. 
% % then features?
% upper footnoot --> notations for different kinds of shape spaces. 
% footnote --> part index or point index
% Feature matrix for 

% \todo{Equiv-net and previous work...}

% \subsection{SE(3)-equivariant Network for Self-supervised Rigid Object Pose Estimation} 
% \subsection{EPN-based Feature Backbone}
% \subsection{SE(3)-equivariant Network and its Use in Self-supervised 6D Pose Estimation for Rigid Objects} 

% \eric{Part-level SE(3) equivariant network design.}
% \subsection{Part-level SE(3)-equivariant Network Design}
\subsection{Part-level SE(3)-equivariant Network}
\label{sec_method_revisit}
% \todo{need to say the pose : from the canonical frame to observed camera frame?}
% \todo{parts, points, rigid transformations}
% \summary{Introduction}
% Part-level SE(3)-equivariant point cloud network $\phi(\cdot, \cdot)$ operates on a point cloud with segmentation labels $X = \{ X_i\vert 1\le i \le K\}$ and part pose $P = \{ P_i \vert 1\le i\le K\}$ for per-part part-level SE(3)-equivariant feature 
% $F = \{ F_i \in \mathcal{F} \vert 1\le i\le K \}$, where $\mathcal{F}$ is an arbitrary feature domain, $K$ is the number of parts. \subsummary{Definition}
% Part-level equivariant feature $F_i$ of part $i$
% Part-level equivariant feature $F_i$ of part $i$ would change equivalently to the rigid transformation part $i$, but invariant to those of other parts. 
% Part-level equivariant feature $F_i$ would change equivalently to the rigid transformation of part $i$, but invariant to that of others. 
% Part-level SE(3)-equivariant point cloud network $\phi(\cdot)$ operates on a segmented point cloud $X$ with per-point pose $P$ for per-part part-level SE(3)-equivariant feature $F = \{ F_i \in \mathcal{F} \vert 1\le i\le K \}$, where $\mathcal{F}$ is an arbitrary feature domain.  \subsummary{Definition}
% \textcolor{myblue}{
We first introduce our part-level SE(3) equivariant network.
% the designed network for per-point part-level SE(3) equivariant feature extraction. 
The network $\phi(\cdot)$ operates on a point cloud 
% $X = \{X_i\vert 1\le i\le N \}$ 
% with 
$X =  \{ \mathbf{x}_i \vert 1\le i\le N \}$ 
with per-point pose and outputs part-level SE(3) equivariant feature 
for each point 
$F = \{\phi(X)[i] \in \mathcal{S} \vert 1\le i\le N \}$, 
where $\mathcal{S}$ is an arbitrary feature domain. 
% $F = \phi(X)[i] \in \mathcal{F} \vert 1\le i\le N \}$, 
% where $\mathcal{F}$ is an arbitrary feature domain.
% $N$ is the number of points in the point cloud. 
% Part-level SE(3)-equivariant point cloud network $\phi(\cdot)$ operates on a segmented point cloud $X = \{ \mathbf{x}_i \vert 1\le i\le N \}$ with per-point pose $P$ for per-point part-level SE(3)-equivariant feature $F = \{ F_i = \phi(X)[i] \in \mathcal{F} \vert 1\le i\le N \}$, where $\mathcal{F}$ is an arbitrary feature domain, $N$ is the number of points in the point cloud. 
% \subsummary{Definition}
Part-level equivariant feature $F_i$ of each point $x_i$ would change equivalently to arbitrary rigid transformation 
% $\in \text{SE(3)}$ 
of the part it belongs to,
% itself, 
but remains invariant to transformations of other parts. 
% others'.
% Part-level equivariant feature $F_i$ of part $i$ would change equivalently to the rigid transformation part $i$, but invariant to those of other parts.
% \subsummary{Property}
% Part-level equivariant feature $F_i$ would change equivalently to the SE(3) transformation applied on it, but invariant to that of others.
% Formally, $\forall A_i\in \text{SE(3)}, 1\le i\le N$, 
% $\forall \{T_{A_i} \vert T_{A_i}: \mathbb{R}^{n\times 3}\rightarrow \mathbb{R}^{n\times 3},  A_i\in \text{SE(3)}, 1\le i\le N\}$, 
Formally, for any set of per-point transformation $\{A_j \in \text{SE}(3) \vert 1\le j\le N \}$ with their corresponding rigid transformations in the spatial domain 
% when transforming points according to their corresponding rigid transformations 
$\{T_{A_j}: \mathbb{R}^{n\times 3} \rightarrow \mathbb{R}^{n\times 3} \vert 1\le j \le N \}$, there is an equivariant transformation $S_{A_i}: \mathcal{S}\rightarrow \mathcal{S}$ for each point $x_i$, 
% $S_{A_i}: \mathcal{F}\rightarrow \mathcal{F}$ 
which only depends on $A_i$ no matter what $A_j$ is applied on other point $x_j (j \neq i)$, such that:
% Formally, $\forall i, 1\le i\le N$, $\forall A_i\in \text{SE(3)}$, there is an equivariant transformation $S_{A_i}: \mathcal{F}\rightarrow \mathcal{F}$, such that $\forall A_j\in \text{SE(3)}, 1\le j\le N, i\neq j$: 
% there are equivariant transformations $\{ S_{A_i} \vert S_{A_i}:  \mathcal{F}\rightarrow \mathcal{F}, 1\le i\le N \}$ so that
\begin{align}
    % \{ S_{A_i} [F_i] \vert 1\le i \le N \} = \phi( \{ T_{A_i} [\mathbf{x}_i] \vert 1\le i \le N \} ),
     S_{A_i} [F_i]  \equiv \phi( \{ T_{A_j} [\mathbf{x}_j] \}_{j=1}^{N} )[i], \forall A_j \in \text{SE}(3). \label{eq_part_equiv_property}
\end{align}
% where 
% $T_{A_j}: \mathbb{R}^{n\times 3} \rightarrow \mathbb{R}^{n\times 3}$
% % $T_{A_i}$ 
% is the corresponding rigid transformation in the input geometry space of $A_j$. 
% Formally, for each part $i$, $\forall A_i\in \text{SE(3)}$, 
% % there  $A, A_i, A_j\in \text{SE(3)}$, 
% there is an equivariant transformation $S_{A_i}: \mathcal{F}\rightarrow \mathcal{F}$ so that
% % $S_A,S_{A_i},S_{A_j}: \mathcal{F}\rightarrow \mathcal{F}$ so that
% % there exists an equivariant transformation $S_A: \mathcal{F}\rightarrow \mathcal{F}$ so that
% \begin{align*}
%     S_{A_i}[\phi(X, P)[i]] = \phi(T_{(A_j)}[X], T_{(A_j)}[P]),
% \end{align*}
% where $T_A: \mathbb{R}^{n\times 3}\rightarrow \mathbb{R}^{n\times 3}, \forall A\in \text{SE(3)}$ is the rigid transformation of a point cloud, $(A_j) = (A_j)_{1\le j\le K}$ denotes SE(3) transformations applied on parts $1,...,K$, $i,j$ are part indexes. 
% $\phi(X, P)[i]$ indicates the output feature for part $i$. 
% \subsummary{Formal property} 
% \zz{What does $\phi(X, P)$ represent?}
% }
% \summary{Approach}
We design 
the network based on the Equivariant Point Network (EPN)~\cite{chen2021equivariant}.
% to seek for such equivariant features. 
The core of our 
% part-level equivariance 
design
% design to achieve \textbf{part-level} equivariance 
is a pose-aware equivariant point convolution module. 
Therefore, in the following text, we would briefly review EPN as a background at first, and then continues with our pose-aware equivarinat point convolution. 
% The core of the design is a pose-aware equivariant point convolution strategy 
% The core of the designed network is a pose-aware equivariant point convolution strategy
% Further, we design a pose-aware equivariant point convolution strategy based on the point convolution proposed in Equivariant Point Network (EPN)~\cite{chen2021equivariant} to seek for such part-level equivariant features. 
% To seek for such part-level equivariant features, we choose Equivariant Point Network (EPN)~\cite{chen2021equivariant} as our base equivariant network and add a pose-aware equivariant feature communication design on the point convolution process of EPN. 
% For each point $\mathbf{x}\in X$, its equivariant feature $\mathbf{f}(\mathbf\x)$ would change equivalently to the SE(3) transformation applied on the part it belongs to, but invariant to that applied on other parts. 
% Formally, 
% \begin{align*}
%     S_{A_i}[\phi(X, P)[\mathbf{x}]] = \phi(T_{(A_j)}[X], T_{(A_j)}[P])
% \end{align*}

% Part-level equivariant pose estimation indicates the estimated part pose for part $i$ to change by the same transformation $A_i$ applied on part $i$ of the input point cloud, i.e. $P_i((T_{A_i})(X)) = T_{A_i}[P_i(X)]$. 
% % For equivariant part pose estimation, we want the estimated pose for part $i$ to change by the same transformation ${A_i}$ applied to the part $i$ of the input point cloud, e.g. $P_i((T_{A_i})(X)) = T_{A_i}[P_i(X)]$. 
% For articulated objects, we also want the estimated pose for part $i$ invariant to the pose change of other parts, i.e. 
% % to be invariant to other parts' pose change, e.g. 
% $P_i((T_{A_j})_{1\le j\neq i\le K}[X]) = P_i(X)$. 
% Combining such two conditions, we can arrive at the condition that equivariant part pose estimation should satisfy: 
% % $P_i((T_{A_j})_{1\le j\le K}[X]) = T_{A_i}[P_i(X)]$.
% $P_i(T_{(A_j)_{1\le j\le K}}[X]) = T_{A_i}[P_i(X)]$.

% Part-level SE(3)-equivariant per-point feature changes equivalently to SE(3) transformation
% Estimating part pose suggests us decompose part poses from part shapes. 
% To make such decomposition easier to conduct, we propose to use Equivariant Point Network (EPN)~\cite{chen2021equivariant}, an SE(3)-equivariant network that achieves equivariance but not at the expense of network expressiveness. 
% Furthermore, we add some special design for point convolution for part-level equivariant features.
% Object pose, as an equivariant property of an object, aligns well with SE(3)-equivariant features, which further suggests the possibility to leverage SE(3)-equivariant networks for object pose estimation. 
% Unsupervised object pose estimation, though as an ill-posed problem, could be made easier by properly extracting invariant/equivariant properties from SE(3)-equivariant features output by EPN~\cite{chen2021equivariant} to design a reconstruction-based self-supervised task~\cite{li2021leveraging}. 
% properly using SE(3)-equivariant features to design a reconstruction-based self-supervised 
% Letting a network predict the invariant object shape and 6D pose at the same time is not an easy thing, especially in an unsupervised manner. 
% Unsupervised pose estimation suggests the network should perform pose and shape decomposition without any use of pose-related annotations. 
% Unsupervised pose estimation suggests the network to decompose object pose from object shape without any access to CAD models,  pose-related annotations, and other supervisions.
% % Unsupervised pose estimation indicates achieving pose and shape disentanglement without any pose realted annotations, known as an ill-posed problem. 
% Known as an ill-posed problem, ~\cite{li2021leveraging} proposes to predict a category-level reference frame for objects in the same category invariant to object pose and estimates the rigid transformation from the reference frame to observed camera space, which could be further treated as the estimated object pose. 
% By observing that object pose is an SE(3)-equivariant property that would be changed by the same SE(3)-transformation $A$ applied to the input point cloud, i.e. $P(T_A[X]) = T_A[P(X)], \forall A\in \text{SE(3)}$, they propose to use SE(3)-equivariant networks, i.e., Equivariant Point Network (EPN)~\cite{chen2021equivariant}, properly to make the decomposition problem simpler. 
% SE(3)-equivariant networks could be properly used to make the decomposition problem simpler. 
% By using features from Equivariant Point Network (EPN) equivariant to a subgroup of SE(3), the decomposition problem could be made simpler. 
% As an ill-posed problem, we can achieve better pose and shape disentanglement leveraging SE(3)-equivariant features~\cite{li2021leveraging}.
% Recently, there is an effort leveraing good properties of SE(3)-equivariant feature extracted by Equivariant Point Network (EPN)~\cite{chen2021equivariant} to do better disentanglement~\cite{li2021leveraging}. 
% For a brief revisit to EPN and how it achieves SE(3)-equivariance. 
% The SE(3)-equivariant network backbone used is Equivariant Point Network (EPN)~\cite{chen2021equivariant}. 

% As a background, we briefly review how EPN achieves SE(3)-equivariance, including rotation equivariance to an arbitrary rotation group element in the SO(3) space, and translation equivariance. 
% \subsummary{Overview}

\vpara{Equivariant Point Network.}
% EPN proposes a kernel-rotated version of KPConv~\cite{thomas2019kpconv} to achieve equivariant transformation in the feature domain. \subsummary{Basic idea}
% %%%% Definition 1 %%%%
% Assume that 
% KPConv extracts a per-point feature $F(X, g)\in \mathbb{R}^{n\times C}$ using the $g$-rotated kernel to perform convolution, where $n$ is the number of points in the point cloud, $C$ is the feature dimension. 
% It satisfies $F(X, g) = F(T_{g^{-1}}[X], \mathbf{1})$, where $T_{g}: \mathbb{R}^{n\times 3}\rightarrow \mathbb{R}^{n\times 3}$ is a rotation transformation induced by the rotation group element $g$. 
% %%%% Definition 1 %%%%
% % Then the convolution using a rotated kernel function satisfies $h_g()$
% %%%% Definition 2 %%%%
% % Specifically, by using KPConv with $g\in \text{SO(3)}$-rotated kernel for feature convolution, we can get features that are equivalent to features extracted by the original KPConv but from the inverse rotation element $g^{-1}$-rotated input, i.e. $g^{-1}X$. 
% %%%% Definition 2 %%%%
% \zz{def. 1 or def. 2?}
% \subsummary{Kernel rotated KPConv}
% EPN proposes a kernel-rotated version of KPConv~\cite{thomas2019kpconv} which outputs a set of per-point features $\mathbf{f}(\mathbf{x}, g)$ equivalent to rotating the input $X$ by $g^{-1}$. 
% Then a per-point feature vector field $F = \{ \mathbf{f}(\mathbf{x}, g) \in \mathbb{R}^C \vert g\in G, \mathbf{x} \in X \}$ equivariant to the rotation group $G$ can be obtained by using each of $g$-rotated KPConv ($g\in G$) for feature processing. 
% \subsummary{Equiv. achieved by using kernel-rotated KPConvs}
% In practice, EPN choose to use the discrete rotation group $G_g$ formed by discretizating the full SO(3) rotation group into 60 different rotations. 
% \subsummary{Implementation}
% Therefore, it extracts a per-point feature field  $F = \{ \mathbf{f}(\mathbf{x}, g) \in \mathbb{R}^C \vert g\in G_g, \mathbf{x} \in X \}$ equivaraint to the discrete rotation group $G_g$. 
% \subsummary{Rot-equiv. property}
% % By discreting the SO(3) rotation group into the icosahedron rotation group $G_g$ containing 60 different rotations, they output a per-point feature vector field $F = \{ \mathbf{f}(\mathbf{x}, g) \in \mathbb{R}^C \vert g\in G_g, \mathbf{x} \in X \}$.
% % xxxx/that will undergo a permutation in the group $G_g$
% % along the dimension $\vert G_g\vert$ 
% % equivariant to each transformation $A\in G_A$ of the input point cloud $X$. 
% % Translation equivariance achieved by EPN is actually translation invariance by using neighbours's relative positions to the target point in the convolution process. 
% % Besides, EPN is translation invariant by using neighbours' relative positions for convolution. 
% Besides, EPN achieves translation equivariance by using neighbours’ relative positions for convolution.
% \subsummary{Translation}
% Combining the above designs, EPN reaches transformation equivariant on a subgroup of the full SE(3) group: $G_A = \{ T_A \vert T_A[X] = T_{\mathbf{t}}T_g[X], \forall \mathbf{t} \in \mathbb{R}^{3}, g\in G_g \}$. 
% % $G_A = \{ T_A\vert T_A[X] = T_{\mathbf{t}}T_g[X], \forall \mathbf{t} \in \mathbb{R}^{3}, g\in G_g (g, \mathbf{t}) \vert g\in G_g, \mathbf{t}\in \mathbb{R}^3 \}$. 
% \subsummary{Equiv. property}
% For computing efficiency, EPN decomposes the full convolution into point convolution and group convolution, where the first design is the key to achieve equivariance. 
% EPN achieves the translation equivariance via translation invariance by using neighbours' relative positions to the target point in the convolution process.
% 
% 
% As a background, we briefly review how EPN achieves SE(3)-equivariance, including rotation equivariance to an arbitrary rotation group element in the SO(3) space, and translation equivariance. 
% \subsummary{Overview}
%%%%% %%%%%
% The key to rotation equivariance is the proposed point convolution strategy leveraging a set of kernel rotated KPConvs 
% for
% % so that it can extract 
% a set of per-point features on which a per-point equivariant feature field could be formed. 
% % \subsummary{Basic idea}
% For an arbitrary rotation element $g$ in the SO(3) space, the $g$-rotated KPConv extracts a per-point feature matrix $F(X, g)$ that is equivalent to the feature matrix extracted by the original version of KPConv but from the inverse element $g^{-1}$-rotated input point cloud. 
% % \subsummary{Rot-equiv. property}
% Formally, $F(X, g)$ satisfies $F(X, g) = F(T_{g^{-1}}[X], \mathbf{1})$, where $T_{g^{-1}}$ is the rotation transformation induced by the rotation element $g$.  
% % \subsummary{Rot-equiv. property}
% % Then, the per-point feature vector field $F = \{ F(X, g) \vert g\in G \}$ equivariant to the group $G$ can be arrived at by using a set of rotated KPConvs formed by rotation elements from a rotation group $G$. 
% Then, by using a set of rotated KPConvs formed by group elements of the rotation group $G$ for per-point feature, we can get a per-point feature vector field $F = \{ F(X, g) \vert g\in G \}$ that is equivariant to rotation group $G$. 
% The translation equivariance of EPN is actually the translation invariance achieved by using relative coordinates for convolution. 
%%%%% %%%%%
EPN takes a point cloud $X$ and a rotation group $G$ as input and extracts per-point per-rotation features $F\in \mathbb{R}^{N\times C\times \vert G\vert}$ that is rotational and translational equivariant to a specific rigid transformation group $G_A$ induced by $G$.
% $G_A = \{ T_{A} = T_{\mathbf{t}} T_{g} \vert g\in G, \mathbf{t}\in \mathbb{R}^3\}$. 
The rotational equivariant transformation for each rotation element $g\in G$ in the feature domain is a corresponding feature permutation of $F$ around the rotation dimension $G$. 
The translational equivariance achieved by EPN is translational invariance by using relative point coordiantes for convolution. %Please refer to EPN~\cite{chen2021equivariant} for more details.
% The per-point feature $F$ would permute along the dimension $G$ in a corresponding way according to the each rotation transformation $g\in G$. 
% When the input point cloud $X$ is transformed 
% The key to rotation equivariance is the proposed multi-rotation point  convolution strategy leveraging multiple kernel-rotated KPConvs. 
% It takes the input point cloud and outputs a per-point equivariant feature field composed of feature vectors corresponding to each rotation element in a specific rotation group $G$. 
% The equivariant feature field would permute in an equivariant manner when the input point cloud has been transformed by a certain rigid transformation. 
% The translation equivariance of EPN is actually the translation invariance achieved by using relative coordinates for convolution.
% Usually, a discrete rotation group $G_g$ is used to design the equivariant feature convolution strategy. 
% Usually, the equivariant feature convolution is designed based on a discrete rotation group $G_g$ for a set of per-point feature vectors corresponding to each rotation element in $G_g$. 
% A common strategy for equivariant property prediction is to predict per-rotation quantity for each rotation group element. 
% Therefore, all predicted properties together are endowed with equivariance. 
% Then, using a set of rotated KPConvs formed by rotation elements from a rotation group $G$ could further lead to a per-point feature vector field $F = \{ F(X, g) \vert g\in G \}$ equivariant to the group $G$. 

% \todo{the name of the design?}
% \vpara{Pose-aware Inter-part Equivariant Feature Communication.}
% \vpara{Pose-aware Equivariant Feature Communication.}
\vpara{Pose-aware Equivariant Point Convolution.}
% Different from object pose estimation, the purpose of this work is to disentangle part poses from part shapes for articulated objects. 
% The part pose estimation goes beyond object pose estimation, aiming for inferring part poses from the input articulated objects. 
% To perform this task, we seek for part-level equivariant features based on EPN by designing a convolution strategy which includes part poses into the feature communication process.
% For rigid objects, we can reduce the effort by reducing the pose range that are needed to be encoded in the feature to the quotient space of each element in the discrete rotation group $G_g$.
% Though equivariant network could produce features that can change equivalently the the pose change of the whole shape, it cannot fulfill our vision, since we also want to disentangle the pose change of contextual parts from the current part's feature learning for those articulated objects. 
% However, for articulated objects, contextual information from adjacent parts would make it harder to disentangle part pose from part shape for the current parts.
% However, for articulated objects, contextual information from adjacent parts would make it harder to disentangle part pose from part shape for the target part due to the 
% Since for , we also want to disentangle the pose change of contextual parts from the current part's feature learning. 
% However, it is possible that contextual information from adjacent parts would make it harder to disentangle part pose from part shape for the current part due to the influence of the pose-related information from other parts. 
% Thus, we propose a convolution strategy by including part poses into the feature communication process of EPN for ``part-level'' equivariant features. 
% to better disentangle pose change of contextual parts from the target part's own features related to its pose and shape information.  
% Thus, given the estimated transformation of each point in the shape canonical space, we propose to include the part pose into the feature communication process of EPN to better disentangle contextual pose information from the part's own feature. 
% To achieve part-level equivariance,
% Simply speaking, 
% we need to consider point pose 
% we communicate features for each point in the local frame where 
% $\vert G_g\vert$ frames where 
% the relative pose between each pair of part is canonicalized.
% EPN features are global equivariant where every points' features would transform in the same way according to the rigid transformation applied on the whole object. 
% % Part-level equivariance cannot be naturally satisfied
% For articulated objects, where articulation variations may lead to different part poses, our part-level equivariance expects that each part feature should be equivariant to its own transforamtion but invariant to others'. 
For part-level SE(3) equivariant features, we design a pose-aware point convolution strategy that operates on a point cloud and per-point poses.
% for feature communication. 
% includes per-point poses for feature  
% We design a pose-aware convolution strategy to arrive at this property. It operates on a point cloud and per-point poses for feature communication. 
% The key idea of the convolution is aggregating neighbours' features with their poses relative to the center point canceled. 
The basic idea is canceling neighbours' relative poses to the center point when communicating features. 
% during the feature communication. 
% in an equviariant manner as if neighbouring points are of same poses to the center point. 
% By saying part-level equivariant feature, we mean that feature should be equivariant to a specific part’s rigid transformation but invariant to others’. 
% To complete this vision, we design a pose-aware point convolution strategy such that during the convolution procedure,
% % during the convolution process, 
% the feature of each point is communicated as if the relative poses of its neighbouring points are canonicalized. 
% % Formally, the designed pose-aware point convolution strategy is as follows:
% % We further propose a pose-aware point convolution strategy for part-level equivariance. \subsummary{Overview}
% % In the convolution process, we wish that point features are communicated as if the relative poses of each point's neighbouring points are canonicalized. 
% \subsummary{Basic idea}
% With estimated part poses, the concept of canonical space and relative canonical states between parts can be naturally defined. 
% Together with the predicted canonical spaces and estimated part poses by the network, 
% % with the estimated part poses and the emerged canonical spaces by the network, 
% we design a pose-aware point convolution strategy to cancel the influence of part pose variations on feature communication. 
% \subsummary{Basic idea}
% Part-level equivariance can be achieved by designing the point convolution strategy such that the point features are communicated as if in each point's local frame where the relative pose between each pair of parts is canonicalized. 
% communicating features for each point in the local frame where the relative pose between each pair part is canonicalized. 
% Based on this 
% idea, we design a pose-aware equivariant point convolution strategy as follows: 
% \textcolor{myblue}{
Formally, taking the per-point pose 
% $P = \{  \mathcal{P}_i \vert 1\le i\le N \}$ 
$P = \{  {P}_i \vert 1\le i\le N \}$ 
and the input point cloud $X$ as input, the 
% designed 
% pose-aware point 
our convolution operator for the point $x_i$'s feature 
% vector 
at the rotation element $g$ is as follows: 
% the designed pose-aware point convolution strategy is as follows:
%%%%% some understandings %%%%%
% That could achieved by inversely transforming the $g$-rotated shape by the relative pose between each contextual part and the current part for each $g\in G_g$. 
% For an intuitive understanding, the estimated part pose could help us define a reference frame where the pose of each part is canonicalized. Then, the feature communication between parts invariant to part pose change could be enforced by communicating features in the reference frame. 
% Then, features equivariant to part $i$'s pose change can be learned based on the reference frame posed by the part pose equivariant to the part pose change. 
% Here, we just project the pose back to the input shape and achieve equivariance from a pose-induced manner to the geometry-induced way.
%%%%% some understandings %%%%%
% Formally, the designed pose-aware equivariant point convolution is as follows:
% feature communication (convolution) is as follows:
% \begin{align}
%   (\mathcal{F}* h_1)(x_i,g) = \sum_{\mathcal{P}_j^{-1}x_j\in \mathcal{N}_{x_i}^c} \mathcal{F}(x_j, g \mathcal{R}\mathcal{R}_j^{-1} ) h_1(g(x_i - \mathcal{P}\mathcal{P}_j^{-1}x_j)), \label{eq_part_level_convolution}
% \end{align}
\begin{align}
  (\mathcal{F}* h_1)(x_i,g) = \sum_{{P}_j^{-1}x_j\in \mathcal{N}_{P_i^{-1}x_i}^c} \mathcal{F}(x_j, g \mathbf{R}_i\mathbf{R}_j^{-1} ) h_1(g(x_i - {P}_{i}{P}_j^{-1}x_j)), \label{eq_part_level_convolution}
\end{align}
where $\mathcal{F}$ is the input function, $h_1(x_i,g): \mathbb{R}^3\times \text{SO}(3)\rightarrow \mathbb{R}^D$ is a kernel, 
% where 
$\mathcal{N}_{P_i^{-1}x_i}^c$ is the set of point $x_i$'s neighbours in the canonical object space, $P_i$ and $P_j$
% $\mathcal{P}_i$ and $\mathcal{P}$ 
denote the input pose of point $x_i$ and point $x_j$ respectively, $\mathbf{R}_i$ and $\mathbf{R}_j$ are their rotation components. 
% }
% respectively. 
% are the input rotations of point $x_i$ and point $x_j$ respectively.  
% \subsummary{Strategy}
% It takes point coordinates and estimated poses as input, further outputs per-point per-rotation point features. 
% Other notations are kept the same to those used in EPN~\cite{chen2021equivariant}.
% The part-level equivariance achieved by this strategy with ground-truth pose
% property 
% could be proved easily, which is deferred to the Appendix. 
% The part-level equivariant property of this convolution strategy with ground-truth pose could be proved easily 
% The part-level equivariant property can be achieved when the estimated per-point pose is accurate. 
% The property can be proved easily, which is deferred to the Appendix. 
% It can be proved easily, which is deferred to the Appendix. 
The proof is deferred to the Appendix.
% It is easy to prove the part-level equivariant property of this point convolution, which is deferred to the Appendix. 
% It is worth mentioning that 
We highlight that 
% \textcolor{myblue}{
we adopt an \emph{iterative pose estimation} strategy. 
Therefore, input poses and rotations in Eq.~\ref{eq_part_level_convolution} are estimated in the last iteration and set to be identities in the first iteration.
% }
%estimated values by the following modules in the last iteration (they are set to identities in the first iteration). 
% values estimated by the following modules in the previous iteration or identities in the first iteration. 
% input point poses and rotations in Eq.~\ref{eq_part_level_convolution} are values estimated by the following modules. 

% \todo{change the statement}
%%%%% %%%%%
% Therefore, our feature backbone takes the input point cloud $X$ and estimated per-point pose $P$ (optional) as input to extract per-point per-rotation feature: ${F}\in \mathbb{R}^{n\times C\times \vert G_g \vert} = \phi(X) = \{ \mathbf{f}(\mathbf{x}, g) \}$, 
% where $\vert \{ \mathbf{x} \} \vert = n$, and $g\in G_g$. 
% \subsummary{A brief summary for the part-level equiv. network}
% % \todo{per-point equivariant feature...}
% The design suggests an iterative part pose estimation approach that feeds part pose and part segmentation estimated in the previous iteration to the next one to participate in the point convolution.
% \subsummary{Iterative}
%%%%% %%%%%
% , in which we feed the estimated part pose from the previous iteration to the next one to participate in the feature convolution process. 
% $\phi(\cdot)$ behaves like EPN in the first iteration.
%%%%% %%%%%%
% For simplicity, we omit the pose-related input and use $\phi(X)$ to denote the feature extraction module in the following text. 
%%%%% %%%%%%
% \subsummary{Notations}
% We will omit the pose-related input to the feature backbone in the notation and simply use $\phi(X)$ in the following text. 
%  the pose-induced equivariant feature computing to the  geometry-induced one. 
% g^{-1}x g^{-1}x_i 
% displacement 
%% here estimated pose = \vert G_g\vert poses...
% Simply speaking, we communicate features for points in each part in the frame as if the articulation states of other parts are canonicalized 
% Simply speaking, point transformation information in the shape canonical space is used to modify the neighbours sampling process and the weight computing process of selected neighbours to the target point. 
% Based on this convolution strategy, we can get features encoding part shape information in the shape canonical shape and residual pose, but invariant to contextual articulation changes. 



% RR_1; RR_2; R_2^T R^T R R_1

% In the above statement, we once mention that the equivariant part feature could be further improved if your have correct part pose parameters that can be further involved in the convolution calculation process. 
% % todos...
% Simply speaking, the idea is to involve the estimated pose into convolution process to disentangle part shapes and part posees between different parts. 
% 

% \subsection{Part-level Equivariance}
% Estimated part poses could be involved in the convolution computation process for better equivariant features that can better disentangle part motions from part shapes. 
% To be more specific, 
% \begin{equation}
%     (\mathcal{F}* h_1)(x,g) = \sum_{x_i'\in \mathcal{N}_{gx}} \mathcal{F}(x - \mathcal{R}\mathcal{R}_i^{-1}x_i', g)h_1(g\mathcal{R}\mathcal{R}_i^{-1}x_i'), 
% \end{equation}
% where $\mathcal{N}_{gx} = \{ g^{-1}(x - \mathcal{R}\mathcal{R}_i^{-1}x_i)\vert x_i\in \mathcal{N}_x \}$ is the set of dispalcements to the neighbours under a rotation $g$ in the canonical space defined by the current point $x$. 
% It can be realized through an articulation mode selection strategy in the convolution process. 

% To perform such invariant feature communication, we need 6D part pose as an additional input to the feature convolution process. That suggests an iterative part pose estimation approach, in which we feed the estimated part pose from the previous iteration to the next one to participate in the feature convolution process. 


% For more details, please refer to~\cite{li2021leveraging} for their self-supervised method and~\cite{chen2021equivariant} for EPN. 

% EPN discretes the SO(3) rotation group into the icosahedron rotation group $G_g$ containing 60 different rotations, and achieve equivariance on a subgrop of SE(3): $G_A = \{ T_A\vert T_A[X] = T_{\mathbf{t}}\circ T_g[X], \forall \mathbf{t}\in \mathbb{R}^3, g\in G_g \}$. 
% EPN achieves equivariance on a subgroup of SE(3), that is $G_A = \{ T_A\vert T_A[X] = T_{\mathbf{t}}\circ T_g[X], \forall \mathbf{t}\in \mathbb{R}^3, g\in G_g \}$, where $G_g$ is the discrete icosahedron rotation group containing 60 different rotations. 
% It proposes a kernel-rotated version of KPConv~\cite{thomas2019kpconv} and outputs a per-point feature vector field $F = \{ \mathbf{f}(\mathbf{x}, g) \in \mathbb{R}^C \vert g\in G_g, \mathbf{x} \in X \}$ using 60 kernel-rotated KPConv networks generated by each rotation element $g\in G_g$.
% The feature field $F$ will undergo a permutation along the dimension $\vert G_g\vert$ equivariant to each transformation $A\in G_A$ of the input point cloud $X$. Note that translation equivariance achieved by EPN is actually translation invariance by using neighbours's relative positions to the target point in the convolution process. 
% Based on EPN, the main idea of~\cite{li2021leveraging} is to let the network propose a category-level canonical frame invariant to SE(3) transformations using SE(3)-invariant obtained by pooling $F$ along the dimension of $G_g$, and predict residual pose for each major rotation $g\in G_g$ from the feature in each $g$'s dimension pooled along the dimension of $X$, e.g. $F^{equiv} = \{ \mathbf{f}^{equiv}(g) \} \in \mathbb{R}^{C\times \vert G_g\vert}$.
% The problem of disentangling object pose from shape can then become much easier since it only needs to achieve this goal on the quotient group $\text{SO(3)}/G_g$. 
% For more details, please refer to~\cite{li2021leveraging} for their self-supervised method and~\cite{chen2021equivariant} for EPN. 
% Although EPN
% Their main idea is to let the network reconstruct a canonical shape invariant to SE(3) transformations using invariant features transformed from equivariant features of the shape, and estimate residual pose for each major rotation 
% For a brief revisit, EPN proposes a kernel-rotated version of KPConv~\cite{thomas2019kpconv} and rotates the kernel by rotations from a finite subgroup $G_g$ of $SO(3)$. 
% Given the input point cloud $X$, each rotated kernel $h_g$ by the rotation element $g$ will result in a new set of per-point features $\mathbf{f}(\mathbf{x}, g)$ satisfying 
% \begin{align*}
%   h_g(\mathbf{x}) = h(T_{g^{-1}}[\mathbf{x}]),
% \end{align*}
% where $\mathbf{x}\in X$, $g^{-1}$ is the inverse rotation of $g$. 
% All rotations $g\in G_g$ will generate a per-point feature vector filed $F = {\mathbf{f}(\mathbf{x}, g)\in \mathbb{R}^C\vert g\in G_g, \mathbf{x}\in X}$, which is rotation equivariant to $G_g$. 
% Transaltion equivariance could be achived by using only relative coordinates in the convolution process. 
% More detailed information could be referred to~\cite{chen2021equivariant}.

% Based on SE(3)-equivariant feature $F = \{ \mathbf{f}(x_i, g_j) \}$ extracted by EPN from the input point cloud $X$, the main idea of~\cite{li2021leveraging} is to let the network propose an invariant shape reference frame $Z\in \mathbb{R}^{N_z \times 3}$ from the invariant feature $F_{inv}$ calcualted from $F$, and predicting object's residual pose $(\Delta \mathbf{R}_g, \Delta \mathbf{t}_g)$ for each rotation hypothesis $g\in G_g$.
% The invariant feature used for canonical shape reconstruction suggesting the consistency across all shapes and SE(3) transformations, as well as $\vert G_g\vert$ redidual pose predictions equivariant to object pose change contribute to the effectiveness of the proposed method together. 

%  indicates that the network should learn to propose a category-level canonical reference frame that is invariant to 6D pose change. 
% However, letting a network predict the invariant object shape and 6D pose at the same time is not an easy thing. 
% The property of equivariant features can facilitate the decomposition of invariant shape and equivariant object pose. 
% Based on the equivariant network, previous work propose to estimate the object's 6D pose by letting the networ predict an invariant category-level reference frame by extracting shape information from invariant feature and further letting the equivariant feature predict the pose-realted equivariant property. 
% EPN can help use generate multiple pose hypothesis based on $\vert G_g\vert$ major pose hypotheses. Then the min-of-N reconstruction loss can make the learning process easier, and at the same time, enforce the network predict a category-level reference frame. 
% \todo{explanation for $G_A$}

% \subsection{Self-supervised 6D Part Pose Estimation}
% \subsection{Motion-based Part-by-part Shape Reconstruction for Articulated Objects}
% \todo{the name of such properties}
% \subsection{Pose Estimation for Articulated Objects}
\subsection{Part Shape, Structure, and Pose Disentanglement}
% \subsection{Articulated Object Pose Estimation}
\label{sec_method_ssl_method}
% Given the point cloud ${X} \in \mathbf{R}^{N\times 3}$ of an articulated object as input and the prior knowledge of the number of parts $K$ for all shapes in the cateogry, the method aims to 
% 1) Reconstruct a category-level reference frame $Z\in \mathbb{R}^{N_z \times 3}$ for $X$ with all parts' pose canonicalized; 
% 2) Estimate the pose $P^i = (\mathbf{R}^i, \mathbf{t}^i)$ for each part $i$ from $Z$ to the observed shape $X$. 
% To perform this task, the network would also naturally decompose the input shape into different parts based on part rigid transformation. 
% Invariant canonical shape reconstruction for articulated objects suggest that the reconstruction should be invariant to all parts' rigid trnasformations.
% Thus, to reconstruct an invariant canonical point cloud $Z$, we propose to reconstruct each part in the canonical space $\{Z_i\}_{1\le i\le K}$ and further assemble them together for the canonical reconstruction of the whole shape.
% Furthermore, to estimate the category-level 6D part pose, we wish that the network should reconstruct part shapes in a category-level canonical reference frame.
% Then, the whole shape is also reconstructed in a category-level canonical space. 
% Moreover, canonical part reconstruction requires the reconstruction to be not only invariant to the pose change of itself, but also invariant to pose changes to its contextual parts. 
% If we do not assume the kinematic constraints between different parts, this suggests that the canonical part shape reconstruction should be invariant to the cartesian product of $K$ SE(3) groups, i.e., $Z_i(\{ X_j \vert 1\le j \le K \}) = Z_i(\{ T_{A_j}(X_j) \vert A_j\in G_A, 1\le j\le K \}), \forall 1\le i\le K$, termed as ``part-level'' invariance. 

% For equivariant part pose estimation, we want the estimated pose for part $i$ to change by the same transformation ${A_i}$ applied to the part $i$ of the input point cloud, e.g. $P_i((T_{A_i})(X)) = T_{A_i}[P_i(X)]$. 
% For articulated objects, we also want the estimated pose for part $i$ to be invariant to other parts' pose change, e.g. $P_i((T_{A_j})_{1\le j\neq i\le K}[X]) = P_i(X)$. 
% Combining such two conditions, we can arrive at the condition that equivariant part pose estimation should satisfy: $P_i((T_{A_j})_{1\le j\le K}[X]) = T_{A_i}[P_i(X)]$.
% Similarly, we call such property ``part-level'' equivariance.
% Thus, we propose a pose-aware inter-part equivariant feature communication strategy to disentangle contextual parts' pose change from the part own equivariant feature learning. 
% It requires per-point pose as additional inputs to perform feature convolution, which suggests an iterative pose estimation procedure. 
 
% Therefore, our feature backbone takes the input point cloud $X$ and estimated per-point pose $P$ (optional) as input to extract per-point per-rotation feature: ${F}\in \mathbb{R}^{n\times C\times \vert G_g \vert} = \phi(X) = \{ \mathbf{f}(\mathbf{x}_i, g_j) \}$, where $\vert \{ \mathbf{x}_i \} \vert = n$, and $g_j\in G_g$. 
% % \todo{per-point equivariant feature...}
% We ommit the estimated pose-related input to the feature backbone in the notation and simply use $\phi(X)$ in the following text.

% Based on the output feature from the backbone, the proposed part-by-part shape reconstruction task is elaborated as follows.

% \eric{Self-supervised disentanglement. We predict four types of information from part-level SE(3) equivariant features including per-part canonical shape $\{  Z_i\vert 1\le i\le K\}$, part-assembling parameters $\{  \mathbf{p}_i^c\vert 1\le i\le K\}$, joint parameters and states $\{ \mathbf{u}_i^j, \mathbf{p}_{i,j}^v, \theta_i^j \}$, and base part 6D transformation $(\mathbf{R}_0, \mathbf{t}_0)$. These information together allow us to reconstruct an input articulated object in a part-by-part manner.}

% To estimate category-level articulated object pose for  articulated objects 
% % in a self-supervised manner
% , 
% we 
% % for articulated objects, 
% % We 
% predict the following three types of information leveraging part-level SE(3)-equivariance:
%%%% %%%%
% To get understanding of the articulated object in an unsupervised manner, we propose to factorize part pose and shape-related information in a hierarchical manner. 
%%%% %%%%
To get a fine-grained understanding of articulated objects, 
% we design a disentanglement strategy that factorizes 
we design a shape, structure, and pose disentanglement strategy.
% for canonical spaces and articulated object pose decomposition.
% to factorize 
% shape and pose-related information at both part-level and object-level. 
To be more specific, 
% given an input articulated object, 
we predict the following three types of information leveraging part-level SE(3)-equivariance from an input articulated object: 
%%%%% %%%%%
% to achieve shape, structure, and pose disentanglement from the input articulated shape:
%%%%% %%%%%
% from part-level SE(3)-equivariant 
% four types of information from part-level SE(3) equivariant 
% features including 
%%%%% %%%%%%%
% 1) \emph{Canonical part shapes}; 
% % $\{  Z_i\vert 1\le i\le K\}$; 
% 2) Object structure, including the \emph{kinematic chain} encoding part adjacency information and transformation order, and \emph{joint parameters} like joint axis directions and pivot points; 
% 3) Articulated object pose, including \emph{part-assembling parameters} that transforms each part from its canonical part space to the canonical object space,
% % the per-part rigid transformation from its own canonical part space to the canonical object space, 
% \emph{joint states} that describes the articulation state of the object
% and a \emph{base part rigid transformation} that transforms the articulated posed shape from the canonical object space to the camera space.
% % from the canonical object space to the camera space. 
% %%%% %%%%
% % Here, we just set the transformation for each from the canonical part space to the canonical object space to a translation vector, called as part-assembling parameters. 
% %%%% %%%%
% % a translation vector for each part's transformation from the canonica
% % 3) Per-part pose from the canonical part space to the observed camera space composed of per-part transformation for part assembling, per-part articulated transformation in the canonical object space, and a part-common rigid transformation from the canonical object space to the observed camera space. 
% % part-assembling parameters $\{  \mathbf{p}_i^c\vert 1\le i\le K\}$, joint parameters and states $\{ \mathbf{u}_i^j, \mathbf{p}_{i,j}^v, \theta_i^j \}$, and base part 6D transformation $(\mathbf{R}_0, \mathbf{t}_0)$. 
% % Those information together allows us to reconstruct the input articulated object in a part-by-part manner.
% The disentanglement is achieved via a part-by-part self-supervised shape reconstruction task. 
% % To predict such part-level information, we first group points into parts 
% Specifically, based on the predicted information, the observed shape is reconstructed by transforming each part from its canonical part space via predicted part-assembling parameters to the canonical object space, then transform each part in the canonical object space via the predicted kinematic chain, joint parameters, and joint states, and further transform the whole articulated posed object by the predicted base part rigid transformation.
% Besides, to better take advantages of part-level equivariance, we add a \emph{part proposal} module which group points to aggregate part-level equivariant features.
% rigid transformation from the canonical object space to the camera space. 
% Specifically, the network reconstructs each part in its canonical part space, and then assembles parts together for the invariant object shape in the canonical object space. 
% After that, each part is transformed in the canonical object space based on predicted kinematic chain, joint parameters and joint states. 
% At last, a part-common rigid transformation is inferred from the ``base part'' defined by the predicted kinematic chain to transform the object from the canonical object space to observed camera space. 
% \zz{how the rigid transformation is predicted and base part? }
%%%%% %%%%%%%
1) {Canonical part shapes}; 2) Object structure; 3) Articulation-aware part rigid transformations.
% Articulated object pose. 
Canonical part shapes are predicted to induce category-level canonical spaces for part pose definition. 
% They ought to be pose invariant.
% The canonical part shape is pose invariant and defined in the corresponding category-level canonical part space.
The object structure contains a kinematic chain that encodes part adjacency information and transformation order, and 
% Among them, object structure contains the \emph{kinematic chain} that encodes part adjacency information and transformation order, and
{joint parameters} such as joint axis directions and pivot points.
% Articulated object pose is composed of three levels of part rigid transformations bridging the proposed canonical spaces and the camera space, that is 1) \emph{part-assembling parameters} that transforms each part from the canonical part space to the canonical object space; 2) \emph{joint states} that describes the articulation state of the object; 3) a \emph{base part rigid transformation} that transforms the articulated posed shape from the canonical object space to the camera space. 
Articulation-aware part transformations include 
% are 
% composed of 
% Articulated object pose is composed of per-part rigid transformations at different levels,
% bridging the proposed canonical spaces and the camera space, 
% that is 
1) {part-assembling parameters} that transform each part from the canonical part space to the canonical object space; 
2) {joint states} that describes the part articulation states in the canonical object space; 
3) a {base part rigid transformation} that transforms the articulated posed shape from the canonical object space to the camera space. 
%The disentanglement 
% is achieved by 
%is learned by
%a part-by-part self-supervised shape reconstruction task. 
% To predict such part-level information, we first group points into parts 
% Specifically, based on the predicted information, the observed shape is reconstructed by transforming each part following three steps: 1) from its canonical part space to the canonical object space via the predicted part-assembling parameters; 2) articulation transformation in the canonical object space; 3) transform the articulated posed object in the canonical object space to the camera space via the predicted base part transformation. 
% Besides, to better take the advantages of part-level equivariance, we add a {part proposal} module which groups points into parts.
% Per-part equivariant features are calculated by aggregating point features. 
Besides, we add a part proposal module for per-part equivariant features to take advantage of part-level equivariance. 
We will elaborate details of the above designs in the following text. 
% a base part is firstly defined from the kinematic chain with the inferred rigid transformation from the canonical object space to observed camera space. 
% Then the predicted base part's transformation is used to transform the posed shape in the canonical object space to the camera space for shape reconstruction. 

% \todo{why we should predict such four types of information?}
% Based on the output part-level SE(3)-equivariant features, we predict four types of information from such features, namely per-part canonical shape, part-assembling parameters, joint parameters and status, and base part 6D pose. 
% To self-supervise the network for such disentanglement, we use shape reconstruction as our self-supervised task and reconstruct the shape in a part-by-part manner based on the predicted part-level properties. 

% Given the predicted information,  we can the get reconstruction of the input shape by  using predicted part-assembling parameters to assemble predicted partxxxxx/ canonical shapes together, inferring joints and changing the articulation state of the reconstructed object based on inferred joint states, transforming the shape via predicted base part pose, to the camera space. 
% To predict such part-properties, we design the model to firstly group points into parts for part-level features, then predict such properties from those features. 
% In the following text, we introduce design details for part-by-part reconstruction. 

% \eric{Explain how these four types of information are used to reconstruct the shape first}

% \eric{Explain how each information gets predicted.}

% In the following text, we introduce the details of the designed invariant shape reconstruction and pose estimation strategy.
% we propose a part-by-part shape reconstruction task to reconstruct 
% we propose a shape reconstruction pipeline that 
% 1) reconstructs the input shape in the canonical space, 2) models part rigid transformations with part kinematics constraint considered, 3) transforms the reconstructed canonical shape to  the camera space to reconstruct the input shape.

% The main idea is to 
\vpara{Part Proposal.}
% \todo{optionally...}
% \eric{With the part-level SE(3) equivariant backbone, we obtain per-point equivariant features.}
% \eric{To further extract part-level features, we introduce a part proposal module.}
% To better perform the part-by-part reconstruction task, we add a part proposal module for shapes with revolute parts for further part-level feature extraction. 
% \eric{This module leverages a grouping function to group input points into $K$ segments so that point features from the same segment can be pooled for part features.}
% The task of this module is to learn a point grouping function $\rho_g$ that maps per-point equivariant feature output by the feature backbone to $K$ clusters. 
% \eric{The grouping function should be SE(3) invariant. Specifically, we leverage an attention-pooling operation together with a slot attention module~\cite{locatello2020objectcentric} for the grouping purpose.}
% \eric{The attention pooling operation extracts per-point invariant features by pooling equivariant features corresponding to different rotation elements.}
% \eric{The slot attention module then consumes the per-point invariant features and learns a point-slot association matrix. Each slot corresponds to a part in our case.}
% With the part-level SE(3)-equivariant backbone, we obtain per-point equivariant features $F$. 
The part proposal module groups points in the input shape $X$ into parts for per-part equivariant features extraction. 
It learns an invariant grouping function that maps $X$ together with the per-point feature $F$ to a point-part association matrix $\mathbf{W}\in \mathbb{R}^{N\times K}$. 
Specifically, we adopt an attention-pooling operation for per-point invariant feature together with a slot attention module~\cite{locatello2020objectcentric} for the grouping purpose.
% The attention pooling operation extracts per-point invariant features $F_{inv} \in \mathbb{R}^{N\times C}$ by pooling equivariant features transformed by a per-point per-rotation MLP from $F\in \mathbb{R}^{N\times C\times \vert G_g\vert}$ corresponding to different rotation elements. 
% The slot attention module then consumes the per-point invariant features and learns a point-slot association matrix. Each slot corresponds to a part in our case.
Based on the proposed parts, we can group points in the input shape $X$ into $K$ point clouds $\{ X_i \in \mathbb{R}^{N_i^p\times 3}\vert 1\le i\le K \}$ and compute per-part equivariant feature matrix $\{ F_i\in \mathbb{R}^{N_i^p\times C\times \vert G\vert} \vert 1\le i\le K\}$, where $N_i^p$ is the number of points assigned to part $i$.
% , where $N_i^p$ denotes the number of points assigned to part $i$.
% Further, per-part equivariant feature matrix can also be computed for grouped parts $\{ F_i\in \mathbb{R}^{N_i^p\times C\times \vert G\vert} \vert 1\le i\le K\}$.
% To further extract part-level features from per-point equivariant feature $F$, we introduce a part proposal module. This module leverages a grouping function to group input points into $K$ segments.
% , with which points features from the same segment can be pooled for part features. 
% so that  point features from the same segment can be pooled for part features. 
% The grouping function should be SE(3)-invariant.
% Therefore, we adopt an attention-pooling operation for per-point invariant feature together with a slot attention module~\cite{locatello2020objectcentric} for the grouping purpose.
% The attention pooling operation extracts per-point invariant features $F_{inv} \in \mathbb{R}^{N\times C}$ by pooling equivariant features transformed by a per-point per-rotation MLP from $F\in \mathbb{R}^{N\times C\times \vert G_g\vert}$ corresponding to different rotation elements. 
% The slot attention module then consumes the per-point invariant features and learns a point-slot association matrix. Each slot corresponds to a part in our case.
% % Based on proposed parts, we can get the per-point equivariant feature and the input point cloud for each part, denoted as $F_i\in \mathbb{R}^{N_i^p\times C\times \vert G_g\vert}$ and $X_i\in \mathbb{R}^{N_i^p\times 3}$ respectively, where $i$ is the part index, $N_i^p$ is the number of points grouped in the part.
% Based on proposed parts, we can get the per-point equivariant feature $F_i\in \mathbb{R}^{N_i^p\times C\times \vert G_g\vert}$ and the input point cloud $X_i\in \mathbb{R}^{N_i^p\times 3}$ for each part by grouping point features together, where $i$ is the part index, $N_i^p$ is the number of points grouped in the part.

% Since we want the learned $\rho_g$ is an invariant function, we first map the per-point 2D equivariant feature to per-point invariant feature vector by pooling the feature along the $G_g$ dimension using attention pooling: $\rho_0: F^{inv} \in \mathbb{R}^{N\times C_{\rho_0}} = \text{Attention-Pooling}_{\mathbf{w}}(\text{MLP}_{\rho_0}(\mathbf{f}(x_i, g_j)\vert \forall x_i\in X, g_j\in G_g))$. 
% % $\rho_0$ could be applied on per-point 2D features for a part $$
% Then, a slot attention module~\cite{locatello2020objectcentric} takes $F^{inv}$ as input and outputs a point-part attention weight matrix: $\rho_{a}: F^{inv}\in \mathbb{R}^{N\times C_{\rho_0}}\rightarrow \mathbf{W}\in \mathbb{R}^{N\times K}$. The summation of each row of $\mathbf{W}$ is equal to $1$, i.e. $\sum(\mathbf{W}[i]) = 1$. 
% We then learn the grouping function by learning a slot-attention module~\cite{locatello2020objectcentric} taking the per-point invariant feature as input and output the attention weight matrix: $\rho_{a}: F^{inv}\in \mathbb{R}^{N\times C_{\rho_0}}\rightarrow \mathbf{W}\in \mathbb{R}^{N\times K}$, with the summation of each the weight matrix $W$'s row $i$ equal to $1$: $\sum(\mathbf{W}[i]) = 1$. 
% where $K$ is a pre-defined value for the number of parts in the category. 
% To make the learned point grouping function invariant to shape global pose change and shape articulation change, we first map the per-point equivariant feature  to per-point SE(3)-invariant feature $F\in \mathbb{R}^{N\times C\times \vert G_g\vert}\rightarrow F_{inv}\in \mathbb{R}^{N\times C}$, and then learn the grouping function by learning a slot-attention module~\cite{locatello2020objectcentric} taking the per-point invariant feature as input: $\rho_g = \text{Slot~Attention}(\text{Attention~Pooling}(F)): F\in \mathbb{R}^{N\times C\times \vert G_g\vert} \rightarrow \mathbf{W}\in \mathbb{R}^{N\times K}$, where $\mathbf{W}\in \mathbb{R}^{N\times K}$ is the point-to-cluster weight matrix with the sum for each of its column to $1$. 
% Given the weight matrix $\mathbf{W}$, each point $i$ is assigned to each cluster by choosing the cluster $j$ in which it has the largest weight $w_{i,j}$.
% Then, each point $i$ is assigned to each cluster by choosing the cluster $j$ with the largest weight $w_{i,j}$ among all $K$ clusters.
% having the largest weight $w_{i,j}$.
% Based on grouped points for each cluster (part), we can get 
% the segmented shape for each part
% the part point clouds,
% proposed part shapes, 
% i.e. $\{ X_i\in \mathbb{R}^{N_i^p \times 3} \vert 1\le i \le K \}$, per-point equivariant feature for each part, i.e. $\{ F_i \in \mathbb{R}^{N_i^p\times C\times \vert G_g\vert} \vert 1\le i \le K \}$, where $N_i^p$ represents the number of points grouped to part $i$. 
% Based on grouped points for each cluster, we can get per-part point cloud, i.e. $\{ X_i\in \mathbb{R}^{N_i^p \times 3} \vert 1\le i \le K \}$, and per-point equivariant feature for each part, i.e. $\{ F_i \in \mathbb{R}^{N_i^p\times C\times \vert G_g\vert} \vert 1\le i \le K \}$, where $N_i^p$ represents the number of points grouped to part $i$. 
% $\rho_0$ could also be applied on the grouped per-point 2D features for a part $i$ or a part pair $i,j$ for their invariant features, i.e. $F_i^{inv}$ and $F_{i,j}^{inv}$ respectively.
% We then further get the input shape for each part, denoted as $\{X_i \in \mathbb{R}^{N_i^p \times 3}\}_{1\le i\le K}$, as well as the per-point equivariant feature for each part, denoted as $\{ F_i \in \mathbb{R}^{N_i^p\times C\times \vert G_g\vert} \}_{1\le i\le K}$, where the upper foot mark $p$ indicates part-level properties.
% change the notation $rho$


% \vpara{Invariant Canonical Shape Reconstruction.}
% \todo{recosntruction or prediction?}
% \vpara{Per-part Canonical Shape Reconstruction.}
\vpara{Shape: Canonical Part Shape Reconstruction.}
% For each part $i$, we learn to predict an invariant canonical shape $Z_i$ from its equivariant feature $F_i$.
% For canonical shape reconstruction, we want to learn an invariant module to reconstruct an invariant reference frame $Z_i$ for each part $i$ based on which the part pose could be defined. 
% Canonical shape reconstructions aims at reconstructing a category-level canonical part shape for each part. 
With per-part equivariant features, 
% and observed part shape, 
we wish to predict a category-level canonical shape for each part to help with the emergence of 
pose-invariant  canonical part spaces of the shape collection.
% category-level part poses. 
% so that expectation for predicting category-level part poses. 
% \subsummary{Why}
% Canonical part shapes should be invariant to all parts’ rigid transformations. 
The canonical shape for each part should be invariant to every parts’ rigid transformations. 
% \subsummary{Overview}
% \subsummary{Property}
% The reconstructed part shape can be treated as the reference frame of the part, based on which the part pose could further be defined. 
% \subsummary{Purpose}
% Such reconstruction for each part requires invariance to all parts' rigid transoformations. 
% \subsummary{Property}
% Therefore, we choose to adopt the same SE(3)-invariant canonical shape reconstruction module as used in~\cite{li2021leveraging}.
Thus, we adopt the same SE(3)-invariant canonical shape reconstruction module as utilized in~\cite{li2021leveraging}
% , which is 
constructed based on an SO(3)-PointNet module. 
% To achieve this goal, we choose to adopt the same SE(3)-invariant canonical shape 
% Specifically, we adopt the same SE(3)-invariant canonical shape reconstruction module as used in~\cite{li2021leveraging}. 
The reconstruction module for each part $i$ takes its equivariant feature matrix $F_i$ and the part coordinate matrix $X_i$ as input and outputs an invariant shape $Z_i\in \mathbb{R}^{N_i^z\times 3}$ with  $N_i^z$ points. 
% where $N_i^z$ is the number of points in $Z_i$.
% The frame of the predicted canonical shape for each part $i$ is then treated as its canonical part space. 
% It takes the equivariant feature matrix $F_i$ and the part coordinate matrix $X_i$ of each part $i$ to extract an invariant shape $Z_i$ leveraging an SO(3)-PointNet. 
% \subsummary{Approach}
% Based on the part-level equivariant feature $F_i$, we choose to use the same SE(3)-invariant canonical shape reconstruction module as used in~\cite{li2021leveraging} achieveing invariance by an SO(3)-PointNet. 


% We propose two kinds of canonical reconstructions: 1) invariant reconstruction for each part in its canonical space, 2) invariant reconstruction for the object in the canonical object space by simply assembling reconstructed parts together by predicting a translation vector for each part from its canonical space to the canonical object space. 
% To let the network perform the above two reconstructions, 
% % Reconstruct each part's invariant shape in its canonical space 
% % To reconstruct the canonical shape invariant to the pose change of each part,
% % % parts' pose variations, 
% % % global pose and part articulation state variations, 
% % we propose to reconstruct an invariant shape for each part in its  canonical space 
% % % canonical shape for each part
% % % each part's invariant canonical shape 
% % and assemble them together for the whole shape's canonical reconstruction. 
% we want to learn two invariant functions for each part: 
% 1) 
% % An invariant 
% An invariant category-level reference frame reconstruction function
% % canonical shape reconstruction function 
% $\rho_i^p: \{F_i\in\mathbb{R}^{N_i^p\times C \times \vert G_g \vert}, X_i \in \mathbb{R}^{N_i^p \times 3} \} \rightarrow Z_i\in \mathbb{R}^{N_i^z\times 3}$. 
% We want $Z_i$ to be invariant to the pose variation of each part, 
% % SE(3) transformations applied on the part change, either caused by the articulation state change of the global pose change, 
% % e.g. $Z_i(\rho_i^p(\phi(X))) = Z_i(\rho_i^p(\phi(T_{\{ A_j \}}[X])))$, 
% % e.g. $Z_i(\rho_i^p(\phi(X))) = Z_i(\rho_i^p(\phi((T_{A_j})_{1\le j\le K}[X])))$, 
% e.g. $Z_i(\rho_i^p(\phi(X))) = Z_i(\rho_i^p(\phi((T_{(A_j)})[X])))$, 
% where $A_j\in \text{SE(3)}$, $i,j$ represents the part index. 
% To achieve the goal of invariant shape reconstruction, we adopt the same SE(3)-invariant canonical shape reconstruction module as used in~\cite{li2021leveraging} based on a SO(3)-PointNet, except that the input to the shape reconstruction module here changes from features of the whole shape to features of a proposed part. 
% 2) An invariant central point prediction function $\rho_i^c: \{F_i\in\mathbb{R}^{N_i^p\times C \times \vert G_g \vert}, X_i \in \mathbb{R}^{N_i^p \times 3} \} \rightarrow \mathbf{p}_i^c\in \mathbb{R}^{1 \times 3}$ that predicts a central point performed as an offset term from its own canonical part space to the canonical object space.
% % from its own canonical reconstruction to the canonical space of the whole shape.
% % \footnote{Central points prediction is necessary for revolute parts only. We put it here since this paragraph aims for whole shape's canonical reconstruction.}. 
% %%%%%%%%%%%%%% --- for approximated invariance and equivariance
% % Considering the approximate SE(3)-equivariance achieved by EPN and context parts' pose change, the learned functions $\{\rho_i^p, \rho_i^c\}$ should be invariant to rotations in the union of $K$ quotient groups $\text{SO(3)}/G_g$. 
% % We still find it an easy problem in practice. 
% %%%%%%%%%%%%%% --- for approximated invariance and equivariance
% After that, the canonical reconstruction for the whole shape 
% % with part associations recovered 
% can be obtained by assembling part reconstructions together via their respective central points, i.e., $Z = \{ Z_i' = Z_i +  \mathbf{p}_i^c \vert 1\le i\le K \}$. 
% % After that, the canonical reconstruction for the whole shape can be obtained by assembling part reconstructions together via their respective central points, i.e. $Z = \{ Z_i = Z_i^c +  \mathbf{p}_i^c \vert 1\le i\le K \}$.
% % \begin{align*}
%   % Z = \{ Z_i +  \mathbf{p}_i^c \vert 1\le i\le K \}.
% % \end{align*}
% Due to the invariance of $\{Z_i, \mathbf{p}_i^c \}$, the reconstructed shape $Z$ is invariant w.r.t. $( A_1,...,A_K), A_i\in \text{SE(3)}, 1\le i\le K$: $Z(\phi(X)) = Z(T_{( A_i )}[X])$.
% % In the following text, we use $Z_i$ to denote the part canonical reconstruction
% % % as the part canonical reconstruction 
% % transformed by its central point $Z_i + \mathbf{p}_i^c$ just for simplicity. 
% %%%%%%%%%%%%%%
% % Given each grouped part $i$, this branch aims to learn a canonical shape reconstruction function $\rho$ that maps per-point features and coordiantes to an invariant point cloud: $\rho: \{F_i\in \mathbb{R}^{N_i^p \times C \times \vert G_g\vert}, X_i \in \mathbb{R}^{N_i^p \times 3}   \} \rightarrow Z_i \in \mathbb{R}^{N_z \times 3}$. 
% % To achieve this goal, we adopt the same SE(3)-invariant canonical shape reconstruction module used in~\cite{li2021leveraging} based on a SO(3)-PointNet, except that the input to the shape reconstruction module here changes from feautres of the whole shape to features of a proposed part. 

% Here, parts are assembled together via their predicted central points.
% Specifically, we wish to learn an invariant  central point prediction function $\rho_i^c: \{F_i\in\mathbb{R}^{N_i^p\times C \times \vert G_g \vert}, X_i \in \mathbb{R}^{N_i^p \times 3} \} \rightarrow \mathbf{p}_i^c\in \mathbb{R}^{1 \times 3}$. 
% Then, the assembled object in the canonical object space is obtained via $Z = \{  Z_i +  \mathbf{p}_i^c \vert 1\le i\le K  \}$. 


% \vpara{Structure: Part-assembling Parameters Prediction.}
% % Part-assembling parameters transform canonical part shapes $\{ Z_i \}$ from their canonical part spaces to the canonical object space. 
% % Aiming for understanding part poses in the object-level with part associations and part kinematics well considered and modeled, we propose to construct a canonical object shape by assembling parts together. 
% % % each part canonical reconstruction $\{ Z_i \}$ from their canonical part spaces to the canonical object space.
% % \subsummary{Purpose}
% % We choose to assemble parts together via rigid transformations. The predicted transformation for each part should be invariant to all parts’ rigid transformations. 
% % \subsummary{Property}
% Part-assembling parameters transform the predicted canonical part shapes such that we can get the canonical object shape
% % canonical object space 
% by assembling the transformed parts together. 
% % The frame of the assembled canonical object shape is then treated as the canonical object space. 
% % from canonical part spaces to the canonical object space. 
% As parameters connecting invariant canonical shapes, they should be invariant to every parts’ rigid transformations as well. 
% Here, we simply predict an offset term $\mathbf{p}_i^c \in \mathbb{R}^{3}$ for each part $i$ that acts as a translation vector between two shapes.
% % connecting two spaces.
% % that transforms the part from the canonical part space to the canonical object space. 
% % The canonical object shape is then formed by assembling those transformed part shapes together.
% % \subsummary{Purpose}
% % to assemble together for the canonical object shape 
% % Based on part canonical reconstructions $\{ Z_i \}$, we assemble those parts together by predicting per-part transformation for part assembling. 
% % We bridge the predicted the canonical part space with canonical object space by predicted per-part transformations. 
% % Therefore, we simply predict an invariant central point $\mathbf{p}_i^c$ performed as a translation vector for each $i$ depicting its location in the canonical object space. 
% Specifically, we view it as an invariant shape reconstruction problem and solve it via an SE(3)-invariant shape reconstruction module~\cite{li2021leveraging} that operates on per-part equivariant feature $\{F_i, 1\le i\le K\}$.
% % by adopting an 
% % and  it via an SE(3)-invariant shape reconstruction module~\cite{li2021leveraging}.
% % The central point prediction problem is treated as an invariant shape reconstruction question and is solved by the an SE(3)-invariant shape reconstruction module~\cite{li2021leveraging}.
% % The central point $\mathbf{p}_i^c$ is predicted from part equivariant feature $F_i$ and part coordinate matrix $X_i$ through the same SE(3)-invariant shape prediction module to that used in~\cite{li2021leveraging}.
% % After that, the object is assembled together by transforming each part from its canonical space to its location in the canonical object space centered at $\mathbf{p}_i^c$: $Z = \{  Z_i' = Z_i +  \mathbf{p}_i^c \vert 1\le i\le K  \}$.
% %%%%%%% how part shapes are transformed and assembled together. 
% %%%%%%% %%%%%%%
% % Then, the canonical object shape can be assembled together by transforming each part from its canonical space to its location in the canonical object space centered at $\mathbf{p}_i^c$: $Z = \{  Z_i' = Z_i +  \mathbf{p}_i^c \vert 1\le i\le K  \}$.
% %%%%%%% %%%%%%%
% % By transforming parts via their corresponding predicted rigid transformations, we can get the assembled object shape, named canonical object space: $Z = \{ Z_i + \mathbf{p}_i^c  \vert 1\le i \le K\}$. 
% % \subsummary{Approach}
% The canonical object shape is formed by assembling parts together $Z = \{ Z_i + \mathbf{p}_i^c \vert 1 \le i\le K \}$.


\vpara{Structure: Kinematic Chain Prediction.}
A kinematic chain defines the part adjacency relationship and part transformation order in the canonical object space, \emph{i.e.} $(i_1,..., i_K)$, where $1\le i_1,...,i_K \le K$ are the indexes of parts. 
% \subsummary{Overview}
% It is important for joint parameters and joint states prediction. 
% the kinematic chain should be an invariant property, not affected by input objects’ articulation state variations. 
The kinematic chain should not be affected by 
% input 
objects’ articulation state variations, and therefore an invariant property.
% \subsummary{Purpose}
% Given the assembled shape, we want to infer part associations, joint parameters and joint states information from it.  
% To arrive at joint parameters, we need to predict adjacent relationship between parts, and the order of their transformation. 
% Thus, we propose to predict a {kinematic chain}, 
% % a sequence of parts depicting the order of part transformation, 
% i.e. $(i_1,..., i_K)$, where $1\le i_1,...,i_K \le K$ are the indexes of parts. 
% The predicted kinematic chain should be an invariant to each part's rigid transformation. 
% The predicted kinematic chain should be invariant to all parts' rigid transformations.
% \subsummary{Property}
% one that would not change if part pose changes.
% Thus, we predict it from per-part invariant features. 
We first construct a confidence graph from object parts and find its 
% a 
maximum spanning tree, 
% from it, 
denoted as $\mathcal{T} = (\mathcal{V}, \mathcal{E}_{\mathcal{T}})$.
The kinematic chain is further predicted as the inverse DFS visiting order of the tree. 
The last part of the predicted kinematic chain is treated as the base part, \emph{i.e.} $i_K$.
%%%%%%%%%%%%%%%%%%%
% Specifically, 
% we first learn an adjacency confidence value from every two parts’ invariant features. 
% % predict an adjacency confidence value $c_{i,j}\in \mathbb{R}$ from each two parts' invariant features. 
% Based on the predicted confidences, we can construct a fully-connected graph with all parts as its nodes and predicted confidence values as edge weights. 
% % using the confidence value as the edge weight. 
% After that, the maximum spanning tree can be found from the constructed weighted graph, denoted as $\mathcal{T} = (\mathcal{V}, \mathcal{E}_{\mathcal{T}})$, where $\mathcal{V}$ is the node set and $\mathcal{E}_\mathcal{T}$ is the weighted edge set of the tree. 
% The inverse DFS visiting order of nodes from the tree is then taken as the predicted kinematic chain.
% % of the input shape. 
% % The base part is taken as the last part of the predicted kinematic chain, i.e. $i_K$.
% The last part of the predicted kinematic chain is treated as the base part, \emph{i.e.} $i_K$.
%%%%%%%%%%%%%%%%%%%
%%%%%% %%%%%%
% Then, a maximum spanning tree $\mathcal{T} = (\mathcal{V}, \mathcal{E}_{\mathcal{T}})$  can be found from the weighted fully-connected graph $\mathcal{G} = (\mathcal{V}, \mathcal{E})$ with parts as its nodes, i.e. $\mathcal{V} = \{ i_1,...,i_K \}$, and predicted confidence values for each part pair $i,j$ as edge weights $w_{i,j}$, i.e. $\mathcal{E} = \{ (i, j, w_{i,j}) \vert 1\le i, j \le K \}$. 
% The inverse DFS visiting order of nodes from $\mathcal{T}$ is then taken as the predicted kinematic chain of the input shape.
% The base part is defined as the last part of the predicted kinematic chain, i.e. $i_K$.
%%%%%% %%%%%%
% \subsummary{Approach}
% \zz{$\mathcal{E}_{\mathcal{T}}$? --- used in the loss function para.}
% Thus, we learn to predict an adjacency confidence value $c_{i,j}\in \mathbb{R}$ from each two parts' invariant features $\{F_{i}^{inv}, F_j^{inv}\}$. 
% Prat invariant feature $F_i^{inv}$ can be obtained by pooling per-point per-rotation feature $\{ \mathbf{f}(\mathbf{x}, g)\vert \mathbf{x}\in X_i, g\in G_g \}$, the same approach to that used in~\cite{li2021leveraging}. 
% % Thus, we learn a function $\rho_{val}$ that predicts an adjacency confidence value from each two parts' ($i$ and $j$) invariant features, 
% % two parts' ($i$ and $j$) invariant features, 
% % i.e. $\rho_{val}: \{ F_{i}^{inv}, F_{j}^{inv} \} \in \mathbb{R}^{2\times C} \rightarrow c_{i,j}\in \mathbb{R}$. 
% After that,
% % we have got the adjacency confidence value for each part pair, 
% a weighted fully-connected graph $\mathcal{G} = (\mathcal{V}, \mathcal{E})$ with parts as its nodes, i.e. $\mathcal{V} = \{ i_1,...,i_K \}$, and predicted confidence values for each part pair $i,j$ as edge weights $w_{i,j}$, i.e. $\mathcal{E} = \{ (i, j, w_{i,j}) \vert 1\le i, j \le K \}$, could be constructed. 
% Then, the kinematic chain is obtained by finding the maximum spanning tree $\mathcal{T} = (\mathcal{V}, \mathcal{E}_{\mathcal{T}})$ from the constructed graph $\mathcal{G}$ and then traversing $\mathcal{T}$ via the DFS algorithm. 
% The inversed visiting order of nodes (parts) of the traversing process is then taken as the predicted kinematic chain of the input shape.






\vpara{Structure: Joint Parameters Prediction.}
% \vpara{Invariant Kinematic Chain Prediction.}
% \todo{for category with more than two parts}
Then, for each adjacent part $(i,j)\in \mathcal{E}_{\mathcal{T}}$, we want to infer their joint parameters, 
% between them, 
including an invariant pivot point $\mathbf{p}_{i,j}^v$ and a joint axis direction hypothesis $\mathbf{u}_i^g$ for each rotation element $g\in G_g$. 
% \subsummary{Overview and purpose}
% $\vert G_g\vert$ joint axis direction hypotheses  $\{\mathbf{u}_i^{g} \}$, where the upper footnote $g$ denotes the group element $g\in G_g$. 
% we predict an invariant pivot point $\mathbf{p}_{i,j}^v$ from their equivariant feature $\{ F_i, Fcor \}$ and coordinate matrices $\{ X_i, X_j \}$.
%%%%% %%%%%
% Firstly, we predict an invariant pivot point $\mathbf{p}_{i,j}^v$ from their equivariant feature $\{ F_i, F_j \}$ and coordinate matrices $\{ X_i, X_j \}$.
% Firstly, we still adopt an invariant shape reconstruction module to predict an invariant pivot point $\mathbf{p}_{i,j}^v$ for each adjacent parts $i,j$ from their equivariant feature $( F_i, F_j )$ and coordinate matrices $(X_i, X_j)$, considering the invariant property required for the pivot point prediction. 
% % using the same invariant function as that for canonical shape reconstruction, \todo{add notation}. 
% After that, we regress 
% % $\vert G_g\vert$ 
% joint axis directions $\{\mathbf{u}_i^{g} \vert g\in G_g \}$ 
% % for rotation matrix or translation scales and translation axis $\{ (\mathbf{u}_i^{g}, s_i^{g})\}$ 
% from each part's equivariant feature $F_i$.
% % for each $g\in G_g$.
% %  depending on the part type of $i$. 
%%%%% %%%%%
For pivot points, we treat them as invariant properties and still adopt an invariant shape reconstruction module for prediction. 
Specifically, we predict the pivot point $\mathbf{p}_{i,j}^v$ between every two adjacent parts $i,j$ from their equivariant feature $( F_i, F_j )$ and the coordinate matrices $(X_i, X_j)$ using an invariant shape reconstruction module~\cite{li2021leveraging}. 
For joint axis directions, we regress an axis direction hypothesis $\mathbf{u}_i^g$ for part $i$ corresponding to each 
% for 
rotation group element $g\in G_g$ from its equivariant feature $F_i$. 
% That is achieved by directly operating $F_i$ via a max-pooling operation over $\{ \mathbf{x}\vert \mathbf{x}\in X_i \}$ followed by an MLP module. 
% \subsummary{Approach}
% \todo{part transformations till now}
%%% move to next para. %%%
% After that, we can get $\vert G_g\vert$ transformation hypotheses for each part $i$ from its canonical part space to the posed shape in the canonical object space. 
% Specifically, for revolute parts, we have $\{ (\mathbf{R}_i^{g} = \mathbf{f}_{\mathbf{R}}(\mathbf{u}_i^{g}, \theta_i^{g}),  \mathbf{t}_i^{g} = \mathbf{R}_i^{g}(\mathbf{p}_i^c - \mathbf{p}_{i,j}^v) + \mathbf{p}_{i,j}^v  )\}$, where $\mathbf{f}_{\mathbf{R}}(\cdot, \cdot)$ maps axis-angle  representation to the rotation matrix. 
% For prismatic parts, we have $\{ ( \mathbf{R}_i^{g} = \mathbf{1},  \mathbf{t}_i^{g} = \mathbf{p}_i^c + s_i^{g}\mathbf{u}_{i}^{g}) \}$. 
%%% move to next para. %%%
% $\pi_i^r: F_i\in \mathbb{R}^{N_i^p \times C\times \vert G_g\vert }\rightarrow \{ \mathbf{q}_i^j, \mathbf{u}_i^j, \theta_i^j \}\in \mathbb{R}^{(4 + 3 + 1)\times \vert G_g\vert}$
 
% Firstly, we need to predict the adjacent relationship between parts. 
% We propose to 
% In the problem setting, we assume that all parts of shapes in one category are with the same type. 
% For prismatic parts, only the translation axis is needed to model for part rigid motion prediction. 
% However, more things related to joints should be recovered for revolute parts such as pivot points between two adjacent parts.  
% That indicates that we should recover the kinematic chain of the input shape, based on which joint-related parameters could be predicted and further part rigid transformations based on the predicted kinematic chain. 
% % For categories whose shapes have more than two parts, we need to predict a kinematic chain from the observed shape to further calculate rigid transformations for each part. 
% % for further rigid part transformation calculation. 
% % The kinematic chain is modeled as a sequence of parts depicting the order of part transformation of the observed articulated shape $(p_{i_1}, ..., p_{i_K})$, where $K$ is the total number of parts in the shape. 
% The kinematic chain is a sequence of parts depicting the order of part transformation of the observed articulated shape, i.e. $(i_1,..., i_K)$, where $1\le i_1,...,i_K \le K$ are the indexes of parts. 
% The 
% This branch is designed for the category whose shapes have more than two parts. Since we have no prior knowledge of the mapping from proposed parts to ground-truth parts, indicating that we have no understanding about the articulation chain between parts proposed by the network, we propose to learn the articulation chain between proposed parts. 
% The predicted kinematic chain should be invariant property that would not change if part pose changes.
% % to object's global pose change and parts' articulation state change.
% Thus, we learn a function  $\rho_{val}$  that predicts an adjacency confidence value from two parts' ($i$ and $j$) invariant features, i.e. $\rho_{val}: \{ F_{i}^{inv}, F_{j}^{inv} \} \in \mathbb{R}^{2\times C} \rightarrow c_{i,j}\in \mathbb{R}$. 
% % For those shapes, we need to predict the connectivity between different predicted parts. 
% % We want to learn a function $\rho_{val}$ that predicts a connectivity confidence value from two parts' ($i$ and $j$) invariant feature: $\rho_{val}: \{ F_{i,inv}, F_{j,inv} \} \in \mathbb{R}^{2\times C} \rightarrow c_{i,j}\in \mathbb{R}^{1}$. 
% % By passing the invariant feature of each part pair, we can get the connectivity confidence value $c_{i,j}$ for each part pair. 
% After that
% % we have got the adjacency confidence value for each part pair, 
% a weighted fully-connected graph $\mathcal{G} = (\mathcal{V}, \mathcal{E})$ with parts as its nodes, i.e. $\mathcal{V} = \{ i_1,...,i_K \}$, and predicted confidence values for each part pair $i,j$ as edge weights $w_{i,j}$, i.e. $\mathcal{E} = \{ (i, j, w_{i,j}) \vert 1\le i, j \le K \}$, could be constructed. 
% Then, the kinematic chain is obtained by finding the maximum spanning tree $\mathcal{T} = (\mathcal{V}, \mathcal{E}_{\mathcal{T}})$ from the constructed graph $\mathcal{G}$ and then traversing $\mathcal{T}$ via the DFS algorithm. 
% The inversed visiting order of nodes (parts) of the traversing process is then taken as the predicted kinematic chain of the input shape.
% Then, we find the largest spanning tree from the constructed fully-connected graph with each node of the graph a predicted part. 
% Further, the articulation chain can then be defined base on the maximum spanning tree. 
% \vpara{Invariant }
% To be more specific, the chain is then defined by traversing the spaning tree from the node having the largest degree via the DFS algorithm. Then, the inverse visiting order of the tree traversal is treated as the articulation chain.  
% \todo{non moving parts from the kinematic chain}

\vpara{Pose: Part-assembling Parameters Prediction.}
% Part-assembling parameters transform canonical part shapes $\{ Z_i \}$ from their canonical part spaces to the canonical object space. 
% Aiming for understanding part poses in the object-level with part associations and part kinematics well considered and modeled, we propose to construct a canonical object shape by assembling parts together. 
% % each part canonical reconstruction $\{ Z_i \}$ from their canonical part spaces to the canonical object space.
% \subsummary{Purpose}
% We choose to assemble parts together via rigid transformations. The predicted transformation for each part should be invariant to all parts’ rigid transformations. 
% \subsummary{Property}
Part-assembling parameters transform the predicted canonical part shapes such that we can get the canonical object shape
% canonical object space 
by assembling the transformed parts together. 
% The frame of the assembled canonical object shape is then treated as the canonical object space. 
% from canonical part spaces to the canonical object space. 
As parameters connecting invariant canonical shapes, they should be 
% invariant to object articulation variations as well. 
invariant to every parts’ rigid transformations as well. 
% Here, we simply predict an offset term $\mathbf{p}_i^c \in \mathbb{R}^{3}$ for each part $i$ that acts as a translation vector between two shapes.
Here, we simply predict a translation vector $\mathbf{p}_i^c \in \mathbb{R}^{3}$ for each part $i$. 
We predict them through invariant shape reconstruction modules from per-part equivariant feature $\{F_i, 1\le i\le K\}$.
% We treat it as an invariant shape reconstruction problem and predict it from per-part equivariant feature $\{F_i, 1\le i\le K\}$. 
% connecting two spaces.
% that transforms the part from the canonical part space to the canonical object space. 
% The canonical object shape is then formed by assembling those transformed part shapes together.
% \subsummary{Purpose}
% to assemble together for the canonical object shape 
% Based on part canonical reconstructions $\{ Z_i \}$, we assemble those parts together by predicting per-part transformation for part assembling. 
% We bridge the predicted the canonical part space with canonical object space by predicted per-part transformations. 
% Therefore, we simply predict an invariant central point $\mathbf{p}_i^c$ performed as a translation vector for each $i$ depicting its location in the canonical object space. 
% Specifically, we view it as an invariant shape reconstruction problem and solve it via an SE(3)-invariant shape reconstruction module~\cite{li2021leveraging} that operates on per-part equivariant feature $\{F_i, 1\le i\le K\}$.
The canonical object shape is formed by assembling parts together $Z = \{ Z_i + \mathbf{p}_i^c \vert 1 \le i\le K \}$.

% \vpara{Base Part 6D Pose Prediction.}
% \vpara{Articulated Object Pose Prediction.}
\vpara{Pose: Joint States Prediction.}
% Based on the predicted kinematic chain, 
% With the predicted part structure
%%%%% %%%%%
% Joint state of a part describes the rotation angle or the translation scalar of each part's transformation along the joint. 
% \subsummary{Overview}
% We choose to predict joint states from each part's equivariant feature to reduce the optimization difficulty. 
% Specifically, for each part $i$, we predict a joint state (a rotation angle $\theta_i^g$ for revolute parts or a translation scalar $s_i^g$ for prismatic parts) for each rotation element $g\in G_g$ from its equivariant feature $F_i$. 
% \subsummary{Approach}
%%%%% %%%%%
Joint states describe the articulation state of an object. 
For each part $i$, we predict a joint state hypothesis for each rotation element $g\in G$ from its equivariant feature $F_i$, \emph{i.e.} a rotation angle $\theta_i^g$ for a revolute part or a translation scalar $s_i^g$ for a prismatic part. By transforming parts in the canonical object space based on the predicted kinematic chain and joint states, we can get the posed articulated shape in the canonical object space. 
% The prediction is performed by directly regressing the equivariant feature $F_i$ through MLPs. 
% With the predicted assembled canonical shape in the canonical object space, the kinematic chain and joint parameters, we further propose to predict the articulated object pose composed of joint states for part articulated transformation in the canonical object space and the base part's rigid transformation from the canonical object space to the camera space. 
% we further predict articulated transformation for each part in the canonical object space, and a part-common rigid transformation to transform the posed shape to the camera space. 
% Then, to transform the posed shape in the canonical object space to the observed camera space without breaking part associations or imposing changes on part articulation states, we propose to infer the 6D pose of the base part.
% To predict part articulated transformation, we predict $\vert G_g\vert$ joint states (rotation angles $\{ \theta_i^{g} \}$ for revolute joints, translation scalars $\{ s_i^{g} \}$ for prismatic joints) for joints between each two adjacent parts $i,j$ in the kinematic chain from the equivariant feature $F_i$ of $i$. 
% Then, for revolute joints, the hypotheses for the transformation around it in the canonical object space
% % its canonical object space to the posed shape in the canonical object space 
% are  $\{ \mathbf{R}_i^{g,o} = \mathbf{f}_{\mathbf{u}, \theta}(\mathbf{u}_i^{g}, \theta_i^g), \mathbf{t}_i^{g,o} = \mathbf{R}_i^{g,o}(- \mathbf{p}_{i,j}^v) + \mathbf{p}_{i,j}^v \}$, where the upper footnote $o$ represents the transformations are in the canonical \textbf{o}bject space. 
% For prismatic joints, we have $\{ \mathbf{R}_i^{g,o} = \mathbf{1}, \mathbf{t}_i^{g,o} =  s_i^{g}\mathbf{u}_i^{g} \}$.

\vpara{Pose: Base Part Rigid Transformation.}
The base part transformation transforms the posed articulated shape in the canonical object space to the camera space.
% \subsummary{Overview}
% The base part is defined as the last part $i_K$ of the predicted kinematic chain. 
We predict a residual rotation hypothesis for each discrete major rotation matrix of the rotation element $g$. 
% corresponding to the rotation element $g$. 
Each residual translation vector is set to zero. 
%%%%%% %%%%%%
% Then, we predict a rotation  matrix $\Delta \mathbf{R}_{i_K}^g$ for each group element $g\in G_g$ from its equivariant feature $F_{i_K}$. 
% % For base part rigid transformation, we first define a base part  as the last part $i_K$ of kinematic chain. 
% % Then, we predict $\vert G_g\vert$ rotation matrices $\{ \Delta \mathbf{R}_{i_K}^{g} \}$ from its equivariant feature $F_{i_K}$. 
% After that, the hypotheses for the base part's rigid transformation are like $\{ (\mathbf{R}^{g} \Delta\mathbf{R}_{i_K}^{g}) , \mathbf{1} \vert g\in G_g \}$, where $\mathbf{R}^g$ is the discrete major rotation matrix of the rotation element $g$.  
%%%%%% %%%%%%
% \subsummary{Approach}

\vpara{Articulated Object Pose.} 
% The articulated object pose can further be calculated based on the above predicted information. 
% \subsummary{Overview}
% Firstly, the rigid transformation of each part $i$ from its canonical part space to the canonical object space is set to its predicted central point $\mathbf{p}_i^c$. 
% Then, the articulated rigid transformation hypotheses of each part $i$ in the canonical object space is calculated 
% % by 
% based on 
% the predicted kinematic chain, joint parameters and joint states. 
% % We denote the predicted hypotheses for each part $i$ as $\{ (\mathbf{R}_i^{g,o}, \mathbf{t}_i^{g,o}) \vert g\in G_g \}$, where $o$ represents the canonical object space. 
% % $o$ denotes the canonical object space. 
% At last, we take the predicted hypotheses for the base part's rigid transformation as the part-common rigid transformation hypotheses.
% % part-common transformation hypotheses. 
% Part pose hypotheses for each part $i$ from its canonical part space to the camera space can be calculated as are denoted as $\{ P_i^g = (\mathbf{R}_i^g, \mathbf{t}_i^g) \}$. 
% % $\{ (\mathbf{R}_i^g = \Delta \mathbf{R}_{i_K}^{g} \mathbf{R}_i^{g,o}, \mathbf{t}_{i}^g = \Delta \mathbf{R}_{i_K}^{g} \mathbf{t}_i^{g,o}) \}$. 
% \subsummary{Approach or components}
With the above predicted quantities, we can calculate per-rotation
articulated object pose hypotheses for an input articulated object $X$, including three parts: 
% % to each rotation group element $g$.
% % for an input articulated object. 
% Specifically, the per-rotation articulated pose 
% % corresponding to each rotation element $g\in G$ 
% is composed of three parts: 
% % The articulated pose of an articulated object is composed of three parts: 
1) rigid transformation $(\mathbf{1}, \mathbf{p}_i^c)$ of each part $i$ from the canonical part space to the canonical object space; 2) per-rotation articulated transformation of each part in the canonical object space computed from the predicted kinematic chain, joint parameters and per-rotation joint states; 3) per-rotation base part rigid transformation from the canonical object space to the camera space. 
% The rigid transformation hypotheses corresponding to each rotation element in the group $G_g$ for each part $i$ from the canonical part space to the camera space are denoted as  $\{  P_i^g = (\mathbf{R}_i^g, \mathbf{t}_i^g) \vert g\in G_g \}$. 
The rigid transformation hypothesis for each part $i$ corresponding to each rotation element $g\in G$
% in the rotation group $G$ 
is denoted as $P_i^g = (\mathbf{R}_i^g, \mathbf{t}_i^g)$. 
We treat them as part pose hypotheses. 
% It is treated
% \zz{Lack of a summary for the predicted articulated pose or the predicted part pose?}
% For instnace, for the revolute part $i$ 
% Based on the above predicted information, for each $g\in G_g$, we can calculate a pose hypothesis for each part from its canonical part space to the camera space based on the predicted part structure and the articulated object pose.
% For each part $i$, we denote its pose hypotheses from its canonical part space to the camera space for each $g\in G_g$ as $\{ (\mathbf{R}_i^g, \mathbf{t}_i^g) \}$, and the hypotheses for its articulated transformation in the canonical object space as $ \{ (\mathbf{R}_i^{g,o}, \mathbf{t}_i^{g,o} )\}$, where $o$ denotes the canonical object space. 

% Specifically, for each part $i$, we have $\{ (\mathbf{R}_i^{g} = \mathbf{R}^g \Delta \mathbf{R}_{i_K}^{g} \mathbf{R}_i^{g,o}, \mathbf{t}_i^{g} = \mathbf{R}^g \Delta \mathbf{R}_{i_K}^{g} \mathbf{t}_i^{g,o}) \}$. 
% Then based on that, the whole shape is transformed from the canonical object space to the camera space.
% % and use its transformation from the canonical object space to the camera space to transform the whole shape. 
% The base part $i_K$ for each object is set to the root part of the spanning tree.
% % the proposed part with the largest number of points. 
% We directly regress its equivariant feature $F_{i_K}$ for $\vert G_g\vert$ quaternions as the rotation representation a $\{ \mathbf{q}_{i_K}^{g} \}$. 
% % Then, its 
% Then, the hypothesis for the base part's transformation for each $g\in G_g$ is calculated as $\{ (\mathbf{R}^{g} \Delta\mathbf{R}_{i_K}^{g}) , \mathbf{1}\}$ 
% % for the pose 
% from the canonical object space to camera space, where $\Delta \mathbf{R}_{i_K}^{g} = \mathbf{f}_{\mathbf{q}}(\mathbf{q}_{i_K}^{g})$, is the rotation matrix that maps the quaternion representation to rotation matrix representation.  
% \todo{pose.. canonical object space.. camera space?}

% Based on those predicted 
% % part-level 
% information stated above
% % for part shapes, part relationship
% , and part pose, we can generate $\vert G_g\vert$ shape reconstruction hypotheses $\{ Y^{g} \}$ for each rotation element $g\in G_g$ 
% by transforming the each reconstructed part $i$ from its canonical part space $Z_i$ to the observed space $Y_i^g$ via predicted transfomrations $\{ ( \mathbf{R}^{g} \Delta\mathbf{R}_{i_K}^{g} \mathbf{R}_i^{g}, \mathbf{R}^{g} \Delta\mathbf{R}_{i_K}^{g}  \mathbf{t}_{i}^{g} ) \}$.
% \todo{formula} 


% \vpara{Equivariant Part Pose Estimation.}
% Then, 
% % In this branch, 
% we wish to estimate the pose of each part from its canonical reference frame to the observed camera space. 
% Similar to the previous approach for rigid object pose estimation, we predict $\vert G_g\vert$ pose hypotheses containing one pose hypothesis $P_{i}^j$ for each $g_j\in G_g$. 
% The part pose estimation strategy defers for different part types. 
% % For revolute part, we choose to use axis-angle revolute representation for part pose prediction to transform the predicted part from its own reference from to the canonical frame of the whole shape. 
% % For revolute part, to model the revolution part transformation, we propose to learn a function $\rho_c$ that predicts a translation vector $\mathbf{p}_i^c$ for each part $i$ to bridge the part canonical space and the shape canonical space from part $i$'s invariant feature: $\rho_c: F_i^{inv}\in \mathbb{R}^{C} \rightarrow \mathbf{p}_i^c\in \mathbb{R}^{3}$. 
% For revolute parts, we propose to learn an invariant pivot point prediction function for each two adjacent parts $(i,j)\in \mathcal{E}_{\mathcal{T}}$: $\rho_{i,j}^v: \{ F_{i,j}^{inv} \} \in \mathbb{R}^{C} \rightarrow \mathbf{p}_{i,j}^v\in \mathbb{R}^{1\times 3}$ for further rigid transformation calculation. 
% Further, a function $\rho_v$ is learned to predict the pivot point $p_{i,j}^v$ for each adjacent parts $i,j$ in the articulation chain for two parts' invariant feature: $\rho_v: \{ F_{i,j}^{inv} \} \in \mathbb{R}^{C} \rightarrow \mathbf{p}_{i,j}^v\in \mathbb{R}^{3}$ to compute part revolute transformation. 
% % The above stated properties are treated as invariant properties 
% % \todo{why they are thought of invariant featuers?}
% The motivation of letting features from two adjacent parts to predict the invariant parameters of the joint between them is to build the relationship between the canonical spaces of such two adjacent parts, and further the relationship between part canonical space and shape canonical space. 
% After that, we predict $\vert G_g\vert$ pose hypothesis containing one 6D pose $P_i^j$ for each $g_j\in G_g$. 
% After that, a residual rotation 
% After that, their part motions in the canonical object space are modeled as rotating around an axis passing through the predicted pivot points. 
% We then factorize the residual rotation matrix $\Delta \mathbf{R}_i^j$ from the axis direction and rotation angle in the canonical space from the per-part equivariant feature $F_i\in \mathbb{R}^{N_i^p\times C\times \vert G_g\vert}$ for each $g_j\in G_g$.
% To do the factorization, we directly predict such properties from $F_i$. 
% Specifically, a function $\pi_i^r: F_i\in \mathbb{R}^{N_i^p \times C\times \vert G_g\vert }\rightarrow \{ \mathbf{q}_i^j, \mathbf{u}_i^j, \theta_i^j \}\in \mathbb{R}^{(4 + 3 + 1)\times \vert G_g\vert}$ is learned, where $r$ represents ``revolute parts'',
% $4$ is for the quaternion representation used in  $\Delta R_i^j$,
% % where $\Delta R_i^j$ uses quaternion representation with the dimension of $4$, 
% $3$ is for the rotation axis direction and $1$ is for the rotation angle.
% Thus, the rotation matrix around the axis for each $g_j \in G_g$ is calculated from the predicted rotation axis direction and angle, i.e. $ \mathbf{R}_i^{j,r} = \mathbf{f}_{\mathbf{u},\theta}(\mathbf{u}_i^j, \theta_i^j)$. 
% Further, the translation vector $\mathbf{t}_i^j\in \mathbb{R}^{3}$ for each $g_j\in G_g$ can then be calculated by
% can be calculated using the corresponding predicted rotation matrix $\mathbf{R}_i^j$, and part pivot point $\mathbf{p}_{i,j}^v$: 
% $\mathbf{t}_i^{j,r} = \mathbf{p}_{i,j}^v - \mathbf{R}_i^j (\mathbf{p}_{i,j}^v - \mathbf{p}_i^c)$. 
% Then, the 
% % $\vert G_g\vert$ 
% pose hypotheses for each part $i$ under each $g_j\in G_g$ 
% are like $\{ P_i^j = (\mathbf{R}_i^j = \Delta \mathbf{R}_i^j \mathbf{R}_i^{j,r}, \mathbf{t}_i^j = \Delta \mathbf{R}_i^j \mathbf{t}_i^j) \}$.
% % After that, 
% for revolute parts, 
% we choose to use axis-angel as part rotation matrix representation
% % we choose the axis-angle representation for part rotation matrix
% $\mathbf{R}_i^j = \{ \mathbf{f}_{\mathbf{R}} (\mathbf{u}_{i}^j, \theta_i^j) \}$ and learn a function $\pi_i: F_i\in \mathbb{R}^{N_i^p \times C\times \vert G_g\vert} \rightarrow \{ \mathbf{R}_i^j \} \in \mathbb{R}^{(3 + 1) \times \vert G_g\vert}$, where $3$ is for rotation axis direction and $1$ for rotation angle. 
% The translation vector $\mathbf{t}_i^j\in \mathbb{R}^{3}$ for each $g_j\in G_g$ can then be calculated by
% % can be calculated using the corresponding predicted rotation matrix $\mathbf{R}_i^j$, and part pivot point $\mathbf{p}_{i,j}^v$: 
% $\mathbf{t}_i^j = \mathbf{p}_{i,j}^v - \mathbf{R}_i^j \mathbf{p}_{i,j}^v$. 
% % We predict rotation angles via predicting values from $0$ to $1$ using a sigmoid function.j

% \todo{angle restriction?}

% Further
% \todo{need to say the details of angle prediction --- from the scale w.r.t. pi to angles?}
% For prismatic parts, we predict the translation axis direction $\mathbf{u}_i^j$, translation scalar $s_i^j$, and the residual rotation matrix $\Delta\mathbf{R}_i^j$ for each part $i$ and each $g_j\in G_g$, i.e.
% % For prismatic parts, we predict $\vert G_g\vert$ translation scalars $\{ s_i^j \}$  along the predicted translation axis 
% % along a predefined axis $\mathbf{u}_p$ and rotation matrix (using quaterion as the rotation representation) for each part $i$: 
% $\pi_i^p: F_i \rightarrow \{ P_i^j = (\mathbf{q}_i^j, \mathbf{u}_i^j, s_i^j) \} \in \mathbb{R}^{N_i^p \times (4 + 3 + 1)\times \vert G_g\vert}$, where $4$ for quaternion, $3$ for translation axis direction, and $1$ for rotation angle. 
% Thus, the per-point per-rot translation can be calculated as 
% % Thus, the per-point per-rot translation can be calculated as
% $\mathbf{t}_i^j = s_i^j \Delta\mathbf{R}_i^j \mathbf{u}_i^j + \mathbf{p}_i^c$. 
% Then, the 
% % $\vert G_g\vert$ 
% pose hypotheses for each part $i$ under each $g_j\in G_g$ are like $\{ P_i^j = (\mathbf{R}_i^j = \Delta\mathbf{R}_i^j, \mathbf{t}_i^j) \}$.
% % then become $\{ P_i^j = (\mathbf{R}_i^j, \mathbf{t}_i^j) \}$.
% Then, the 6D pose hypothesis $P_i^j$ for each part $i$ for each rotation $g_j\in G_g$ is $\{ P_i^j = (\mathbf{R}_i^j, s_i^j\mathbf{R}_i^j \mathbf{u}_p) \}$. 
% In practice, to make the rotation/translation axis direction and $\Delta \mathbf{R}_i^j$ the same for each part, we set such properties of all parts to the predicted ones of the part with the largest number of point. 

% Together with the discrete major rotation matrix $\mathbf{R}_g^j$ of each $g_j\in G_g$, we can get $\vert G_g\vert$ pose hypotheses for each part $i$, i.e.
% % $\{ P_i^j = (\mathbf{R}_g^j\mathbf{R}_i^j, s_i^j\mathbf{R}_g^j \mathbf{R}_i^j \mathbf{u}_p) \}$.
% $ \{ P_i^j = (\mathbf{R}_g^j \mathbf{R}_i^j, \mathbf{R}_g^j \mathbf{t}_i^j) \} $.


% translation vectors $\{ \mathbf{u}_i^j \}$ and translation scalars $\{ s_i^j\}$ for each part $i$: $\pi_i: F_i\in \mathbb{R}^{N_i^p \times C\times \vert G_g\vert} \rightarrow \{ \mathbf{R}_i^j \} \in \mathbb{R}^{(3 + 1) \times \vert G_g\vert}$, where $3$ is for the translation axis direction and $1$ for translation scalar. 
% % For prismatic parts, we predict $\vert G_g\vert$ scalars $\{ s_i^j \} \in \mathbb{R}^{1 \times \vert G_g\vert}$ as translation scales along a predefined translation axis direction $\mathbf{u}_p$ for part translation vector calculation as the part pose representation: $\pi: F_i\in \mathbb{R}^{N_i^p\times C\times \vert G_g\vert } \rightarrow \{ s_i^j\mathbf{u}_p \} \in \mathbb{R}^{3\times \vert G_g \vert}$. 
% Then, the 6D pose hypothesis $P_i^j$  for each part $i$ for each $g_j \in G_g$ is represented as $\{  P_i^j\} \in \mathbb{R}^{(9 + 3) \times \vert G_g\vert} = \{  \mathbf{R}_i^j, s_i^j \mathbf{R}_i^j \mathbf{u}_i^j \}$. 

% Then, together with the discrete major rotation matrix $\mathbf{R}_j^g$ of each element $g_j\in G_g$, we can get the 6D pose hypothesis for each part $i$: $\{ P_i^j \} \in \mathbb{R}^{(9 + 3)\times \vert G_g\vert}  = \{ (\mathbf{R}_j^g\mathbf{R}_i^j, \mathbf{R}_j^g\mathbf{t}_i^j) \}$. 

% \todo{prismatic parts}

\subsection{Shape Reconstruction-based Self-supervised Task}
% \subsection{The Self-supervised Task}
\label{sec_method_self_supervised_task}
% \todo{something for the task...}
Based on the reconstructed canonical part shape and predicted per-rotation part pose hypothesis, we can get per-rotation shape reconstruction for each part $i$: 
% the per-rotation reconstructed shape for each part $i$: 
$\{ Y_i^{g} = \mathbf{R}_i^g Z_i + \mathbf{t}_i^g \vert g\in G\}$. 
% \subsummary{Part reconstruction}
% Based on the predicted per-part per-rotation part pose, we can get per-rotation reconstructed shape for each part $i$: $\{ Y_i^{g} = \mathbf{R}_i^g Z_i + \mathbf{t}_i^g \}$. 
% Based on the per-rotation reconstructed shape, 
% Then based on those reconstructed part shapes, we use a shape reconstruction task to self-supervise the network's learning process. 
% Besides, some regularizations are added for predicted joints. 
% joint prediction. 
% Further, we adopt a part-by-part reconstruction task to self-supervise the network.
A part-by-part reconstruction task is adopted to self-supervise the network. 
% 's learning. 
Besides, 
we add a regularization term for predicted joints to make them behave like real joints. 
% some regularization terms are added for predicted joints. 

% \zz{per-rotation?}

\vpara{Shape Reconstruction-based Self-supervised Loss.}
% Using the method proposed in~\cite{li2021leveraging}, we first estimate the pose $(\mathbf{R}_{glb}, \mathbf{t}_{glb})$ of the input shape $X$ by  treating it as a rigid object for better performance.
% Together with $(\mathbf{R}_{glb}, \mathbf{t}_{glb})$, we can get a 6D pose hypothesis for each part $i$ for each 
% $g_j \in G_g$ from the proposed invariant canonical space to the observed camera space: 
% $ \{ P_i^j  = (\mathbf{R}_{glb} \mathbf{R}_g^j \mathbf{R}_i^j, \mathbf{R}_{glb}\mathbf{R}_g^j \mathbf{t}_i^j)\} $.
% $ \{ P_i^j \} \in \mathbb{R}^{(9 + 3) \times \vert G_g\vert}$. 
% $g_j\in G_g$: $\{ P_i^j = (\mathbf{R}_{glb} \mathbf{R}_g^j \mathbf{R}_i^j, ) \}$
% todo: xxx
% After we have got $G_g$ part pose hypotheses for each part, 
% Then 
The per-rotation shape reconstruction for the whole object can be calculated by concatenating all part reconstructions: 
$Y^{g} = \{ Y_i^{g} \vert 1\le i\le K \}$.
% $Y^{g} = \{ Y_i^{g} \}_{1\le i\le K}$. 
% \subsummary{Per-rot reconstruction}
% For each $g \in G_j$, the whole shape can be reconstructed by concatenating all part reconstructions: 
% we can get the reconstructed whole shape by concatenating all part reconstructions: 
% $ Y^{g} = \{ Y_i^{g} \}_{1\le i\le K}$.
% $Y^j = \bigcup_{1\le i \le K}\{ Y_i^j = \mathbf{R}_i^j Z_i + \mathbf{t}_i^j \}$. 
We then adopt a min-of-N loss between the input observation $X$ and the reconstructed posed point clouds: 
\begin{align}
    \mathcal{L}_{rec} = \min_{ g \in G } d(X, Y^{g}),  \label{eq_recon_loss}
\end{align}
where $d: \mathbb{R}^{N_X\times 3} \times \mathbb{R}^{N_Y\times 3}\rightarrow \mathbb{R}$ denotes the distance function between two point clouds. 
% Assume that the minimum reconstruction error is achieved by the reconstructed object of the 
% \subsummary{Loss}
% The same to~\cite{li2021leveraging}, 
% The same to~\cite{li2021leveraging}, Chamfer Distance function is used for complete point clouds, while unidirectional Chamfer Distance is used for partial point cloud. 
% denotes the distance function between two point clouds. 
% We choose the Chamfer Distance function for complete point clouds, while a unidirectional Chamfer Distance is used for partial point cloud, where only the distance form the observed shape to reconstructed shape is used to calculate the reconstruction loss.
% The same to~\cite{li2021leveraging}, we choose the Chamfer Distance fucntion for full observed point cloud, while a unidirectional Chamfer distance is used for partially point cloud input, where only the distance from observed shape to shape reconstruction is used for further shape reconstruction loss calculation. 

% to further predict the part revolute transformation, we need to predict the rotation matrix 
% $\mathbf{R}_i$ and the translation vector $\mathbf{t}_i$ for each part $i$. 
% Here, we choose the axis-angle representation for part rotation matrices 
% Here, we choose to use the aixs-angle representation for part rotation matrix $\mathbf{R}_i = {\mathbf{f}}_{\mathbf{R}}(\mathbf{u}_{i,j}, \theta_i)$. 
% The translation vector for the part $i$ is computed based on the predicted translation vecotr $\mathbf{p}_i^c$, pivot point $\mathbf{p}_{i,j}^v$ and the 
% Then, for each pair of parts $i,j$, 
% That means that we need to predict 
% Here, we choose the axis-angle representation for part pose of each part. 
% % todo: motivation for axis-angle representation?
% We therefore propose to learn a function $\pi: F_i^p \in \mathbb{R}^{N_i^p\times C\times \vert G_g\vert} \rightarrow \{ P_{i,j}^p \}\in \mathbb{R}^{(3 + 1) \times \vert G_g\vert}$, where $3$ is for axis direction, and $1$i is for angle as our rotation representation. 



% The function $\rho$ is invarint 
% the global rotation matrix and $\mathbf{}$
% reconstruct an invariant shape point cloud $\mathbf{Z}_i\in \mathbb{R}^{N_z\times 3}$ for each part $i$; 2) reconstruct an invariant shape point cloud $\mathbf{Z}\in \mathbb{R}^{N_pN_z\times 3}$ for the whole shape by transforming each canonical part reconstruction via its articulation 
% In order to decompose the shape into parts with part shape and part pose decomposed for each of them, we adopt a rigid motion-based part-by-part reconstruction self-supervised task to self-supervise the network's learning process. 
% To facilitate the part pose-shape decomposition process, we predict shape for each part in its own canonical space, and then transform the canonical reconstruction to the observed camera space via predicted rigid transformation. 

% To further model part rigid transformation based on joint parameters, we decompose the transformation from part canonical space to observed camera space into three transformation steps: 
% 1) Transform part shape from its own canonical space $\mathbf{P}_i^{PC}$ to the shape canonical space; 2) Transform the part shape in the shape canonical space via predicted rigid transformation to the part shape in shape canonical space $\mathbf{P}_i^{SC}$; 3) Transform the part shape in the shape canonical space to the observed camera space $\mathbf{P}_i$ via a rigid transformation same for all parts. 
% The main goal is to treat each part in the observed camera space as a rigid object transforming from the part canonical space to the observed shape. 
% Moreover, we also use a 
% todo: previous similar strategies?
% A common strategy for part decomposition in previous works is predicting parts from a common shape feature~\cite{chen2019bae,kawana2022uppd}. 
% In this method, we add a point grouping module to group points for part proposal to further generate part features based on point grouping result for better part shape and pose decomposition. 
% Thus, the main method is composed of 1) A part proposal module to group points into different clusters; 2) A part motion prediction module to predict part motions from equivariant features based on grouped point features for each part. To put the part motion into a real senario, we model part motions by predicting joint parameters and joint-aware motion parameters. 
% state here or in the supp?
% We assume that we have the prior knowledge of the number of parts for shapes in one specific category. 
% Thus, for categories with more than two parts, an articulation chain is needed to be predicted based on the grouped clusters. 
% After that, joint parameters are predicted based on part adjacency prediction. 
% % This enables us to predict part motions and part adjacency
% Besides, to better disentangle contextual articulation information from a part's shape and pose related information, a part-aware inter-part feature communication strategy is proposed to encourage part features to be invariant to contextual articulation change. 
% % Besides, to better ``treat a part as a rigid object'', an SE(3)-invariant feature communication strategy is designed to facilitate inter-part invariant shape feature exchange. 
% The method makes no assumption on the alignment or any other prior knowledge on the orientation of input shapes. In practice, we use add a global alignment module to align input shapes at first for better performance. 
% % chain prediction? ---- how to get a chain...?
% % 

% \subsection{Equivariant Point Network}
% Considering arbitrary poses of the input shape, equivariant point network is used to process the input shape for shape features equivariant to global pose variations: $\{\mathbf{H}_{i_p}\}_{i_p\in [N]} = \text{EPN}(\mathbb{S})$, where $\mathbf{H}_i\in \mathbb{R}^{\vert G\vert \times C}$, $N$ is the number of points in the input shape, $G$ is the discrete rotation group, $C$ is the dimension of point features. 
% % Specifically, the output feature $\mathbf{H}$ 

% Different from~\cite{li2021leveraging}, where only the global pose is needed to be factorized from the input shape, we wish to factorize the pose and shape for each individual part. 
% Thus, we design a strategy to get better part equivariant features with shape context information preserved but motion information disentangled. This could be done by changing feature communication strategy. 

% \subsection{Slot Attention-based Part Proposal}
% % better part motion attributes prediction
% To complete the part-by-part motion-based reconstruction task better
% A slot attention~\cite{locatello2020objectcentric} module is used to group points in the input shape, taking point invariant features pooled from output point equivariant features:
% \begin{align}
%     \mathbf{h}_i &= \text{Attention~Pooling}(\mathbf{H}_i) \\ 
%     \mathbf{W} &= \text{Slot~Attention}(\{ \mathbf{h}_i \}_{i\in [N]} ),
% \end{align}
% where $\mathbf{W} \in \mathbb{R}^{N\times K}$ is the attention weight matrix from points to different slots. 

% After that, we can get part-level features for part-level properties prediction based on point grouping result obtained by the above part proposal strategy.
% To be more specific,
% \begin{align}
%     \mathbf{H}_i^{P} &= \text{Attention~Pooling}(\text{MLP}(\{ \mathbf{H}_{i_p}  \}_{{i_p}\in \hat{\mathbb{S}}_i } )) \\ 
%     \mathbf{h}_{i}^{P} &= \text{SO(3)-PointNet}(\mathbf{P}_i, \text{MLP}(\{ \mathbf{H}_{i_p} \}_{i_p \in \hat{\mathbb{S}}_i})),
% \end{align}
% % where $\mathcal{N}_i$ is the point set of the part $i$, 
% where $\mathbf{H}_i^{P}$ is the equivariant feature matrix the part $i$, $\mathbf{h}_{i}^{P}$ denotes the part-level invariant features. 
% Similarly, we can predict such features for two part shapes via:
% \begin{align}
%     \mathbf{H}_{i,j}^{P} &=  \text{Attention~Pooling}(\text{MLP}(\{ \mathbf{H}_{i_p}  \}_{{i_p}\in \hat{\mathbb{S}}_i \bigcup \hat{\mathbb{S}}_j } )), \\
%     \mathbf{h}_{i,j}^{P} &= \text{SO(3)-PointNet}(\mathbf{P}_i, \mathbf{P}_j, \text{MLP}(\{ \mathbf{H}_{i_p} \}_{i_p \in \hat{\mathbb{S}}_i \bigcup \hat{\mathbb{S}}_j})).
% \end{align}



% \subsection{Part Rigid Motion Prediction}
% \subsection{Part-by-part Motion-based Shape Reconstruction}
% % articulation chain prediction --> the step to get part connection relationshi
% % Part motion information is used to
% % A motion-based part-by-part reconstruction strategy is used to decompose part shape from
% To infer part pose from the observed shape, we predict the observed part by 1) predicting its shape in its own canonical space, 2) transforming it to the shape canonical space, 3) transforming the part shape in the shape canonical space via part-specific rigid transformation $\{ \mathbf{R}_i^{C}, \mathbf{t}_i^{C} \}$, 4) transforming the part shape from the shape canonical space to observed camera space via a common global rigid transformation $\{ \mathbf{R}_{glb}, \mathbf{t}_{glb}\}$. 
% % The rigid motion for each part $i$ from its own canonical space to the observed camera space is decomposed to the part-specific rigid motion $\mathbf{R}_i^{C}, \mathbf{t}_i^{C}$ from the part canonical space to shape canonical space, and a common rigid motion $\mathbf{R}_{glb}, \mathbf{t}_{glb}$ from the shape canonical space to the camera space for all parts. 
% Below we first introduce how to predict part-specific rigid transformations, and then the global rigid transformation common for each part.
% Based on the articulation chain, which defines the connection relationship among parts, we predict part rigid transformation by predicting joint parameters between two parts and the revolute or prismatic transformation along the joint. 
% First, part $i$'s shape in its own canonical space $\mathbf{P}_i^{PC}$ is predicted from its invariant feature: 
% \begin{align}
%      \mathbf{P}_i^{PC} &= \text{MLP}(\mathbf{h}_i^{P}).
% \end{align}
% Then for revolute parts, two invariant properties, namely the central point $\mathbf{p}_i^{c}$, and the pivot point $\mathbf{p}_{i,j}^{v}$ between part $i$ and its adjacent part $j$, are predicted from corresponding part invariant features: 
% \begin{align}
%     \mathbf{p}_i^{c} &= \text{MLP}(\mathbf{h}_i^{P}) \\ 
%     \mathbf{p}_{i,j}^{v} &= \text{MLP}(\mathbf{h}_{i,j}^{P}).
% \end{align}
% % We predict a part $i$ in the shape canonical space $\mathbf{P}_i^{PC}$ by predicting the shape in its own canonical space, a central point for this part in the shape canonical space, and a revolute transformation based on its predicted joint parameters. 
% % Part shape in the part canonical space, central point are considered as invariant properties and predicted from the part's own invariant feature:
% % \begin{align}
% %     \mathbf{P}_i^{PC} &= \text{MLP}(\mathbf{h}_i^{P}) \\ 
% %     \mathbf{p}_i^{c} &= \text{MLP}(\mathbf{h}_i^{P}).
% % \end{align}
% % The pivot point $\mathbf{u}_{i,j}$ between two adjacent parts $\mathbf{P}_i^{SC}, \mathbf{P}_j^{SC}$ is also considered as an invariant property and is regressed from two parts' invariant feature: 
% % \begin{align}
% %     \mathbf{p}_{i,j}^{v} = \text{MLP}(\mathbf{h}_{i,j}^{P}).
% % \end{align}
% Then two equivariant features, namely joint axis direction $\mathbf{u}_{i,j}$ and the rotation angle $\theta_{i,j}$, are regressed from the two-dim part equivariant feature matrix to describe the revolute transformation for parts in the canonical space of each discrete element $g$: 
% % The axis direction $\mathbf{u}_{i,j}$ and rotation angle $\theta_{i,j}$ are considered as equivariant features and are regressed from two-dim part feature matrix:
% \begin{align}
%     \mathbf{U}_{i,j} &= \text{MLP}(\mathbf{H}_i^{P}) \\ 
%     \Theta_{i,j} &= \text{MLP}(\mathbf{H}_i^{P}),
% \end{align}
% where $\mathbf{U}_{i,j}\in \mathbb{R}^{\vert G\vert \times 3}$ is the axis direction matrix with each of its row an axis vector of unit norm for a rotation group element, $\Theta_{i,j} \in \mathbb{R}^{\vert G\vert}$ is the rotation axis angle matrix with each of its element an angular value. 
% Then, the part shape in the shape canonical space of each rotation group element $g$ is predicted by transforming the predicted part shape in the part canonical space to the shape canonical space: 
% \begin{align}
%     \mathbf{P}_i^{SC} = \mathbf{R}_i^{C}[g](\mathbf{P}_i^{PC} + \mathbf{p}_i^{c}) + \mathbf{t}_i^{C}[g],
% \end{align}
% where $\mathbf{R}_i^{C}[g]$ and $\mathbf{t}_i^{C}[g]$ are the rotation matrix and translation vector of the rotation group element $g$, respectively. They are calculated by transforming the predicted axis direction and rotation angle, together with the predicted pivot point: 
% \begin{align}
%     \mathbf{R}_i^{C}[g] &= \mathcal{F}_{\mathbf{R}}(\mathbf{U}_{i,j}[g], \Theta{i,j}[g], \mathbf{p}_{i,j}^{v}) \\ 
%     \mathbf{t}_i^{C}[g] &= \mathcal{F}_{\mathbf{t}}(\mathbf{U}_{i,j}[g], \Theta{i,j}[g], \mathbf{p}_{i,j}^{v}).
% \end{align}

% % % two steps
% % % todo: how to get part equivariant feature and invariant feature
% % The part in the observed space is modeled by transforming part shapes in the canonical space via rigid transformations. To put the part motion into a real senario, part motion is further decomposed to a revolute or prismatic motion and further a global rotation. For revolute part motion, we let the part equivariant feature predict a unit vector $\mathbf{u}$ as the residual axis direction. Also, we predict a pivot point in the shape canonical space for each joint from its two adjacent parts:
% % \begin{align}
% %     \mathbf{h}_{i,j} &= \text{SO(3)-PointNet}(\{\mathbf{H}_{i_p}\}_{{i_p}\in \mathcal{S}_i \bigcup \mathcal{S}_j}, \mathbf{P}_i, \mathbf{P}_j) \\ 
% %     \mathbf{q}_{i,j} &= \text{MLP}(\mathbf{h}_{i,j})
% % \end{align}
% % % todo: axis prediction from equiv-feature
% % % 
% % Then, the revolute part motion in the shape canonical space is modeled as a revolution transformation: $\mathbf{P}_i^{S} = \mathbf{R}_i^{S}\mathbf{P}_i^{P} + \mathbf{t}_i^{P}$, where $\mathbf{R}_i^{S} = \mathcal{F}_{\mathbf{R}}(\mathbf{u}_i, \mathbf{q}_i)$, is the rotation matrix of part $i$ calculated from the predicted joint axis direction $\mathbf{u}_i$ and the joint pivot point $\mathbf{q}_i$, $\mathbf{t}_i^{S} = \mathcal{F}_{\mathbf{t}}(\mathbf{u}_i, \mathbf{q}_i)$ is the translation vector of part $i$. 

% \vpara{Prismatic parts.} For prismatic parts, we fix the part axis $\mathbf{u}_i$ for each part $i$ and predict the translation vector $s_i$ for each part along $\mathbf{u}_i$ in the part canonical space under each rotation group element $g$: 
% \begin{align}
%     \mathbf{S}_i = \text{MLP}(\mathbf{H}_i^{P}),
% \end{align}
% where $\mathbb{S}_i\in \mathbb{R}^{\vert G\vert \times 1}$ is the translation matrix. 
% Then, the prismatic part's transformation from the part canonical space to the shape canonical space under each rotation group element $g$ is: 
% \begin{align}
%     \mathbf{P}_i^{SC} = \mathbf{P}_i^{PC} + \mathbf{S}_i[g]\mathbf{u}_i.
% \end{align}

% After that, a global rotation matrix $\mathbf{R}_{glb}$ is selected from the discrete rotation group $G$ such that the reconstruction chamfer distance of the predicted shape transformed from shape canonical space to the camera space under $\mathbf{R}_{glb}$ is the smallest one. 
% For complete shapes, the center of input shape is used directly as global translaton $\mathbf{t}_{glb} = \overline{\mathbf{P}}$, while for partial input shapes, the translation vector is predicted from the corresponding shape feature for each rotation group element $g$. 
% % Prismatic parts' transformation are modeled by translating a part along a predefined axis direction $\mathbf{u}_i$: $\mathbf{t}_i = s_i \mathbf{t}_i$, where $s_i$ is the length of the predicted part translation. 

% % Part motions from the canonical space of each part to the observed space is then modeled by the part transformation from part canonical space to shape canonical space, followed by a global shape rotation matrix $\mathbf{R}_{glb}$. 
% % \begin{itemize}
% %     \item Strategy: along the joint, global rotation
% % \end{itemize}

\vpara{Regularization for Joint Prediction.}
% \subsection{Constraints for Joint Prediction} \label{sec_method_joint_prediction}
% One challenging thing of part motion modeling in the canonical space is how to predict the joint $\mathbf{u}_{i,j}$ between two parts $\mathbb{S}_i, \mathbb{S}_j$. 
% In this method, we predict the joint between two adjacent parts $i,j$ by predicting the joint direction $\mathbf{u}_{i}$ and a pivot point $\mathbf{p}_{i,j}^v$. 
% Predicted joints should behave like real joints for 1) predicting ``real’’ part articulated transformations in the canonical object space, and 2) part-level equivariant features that are more likely output by the pose-aware point convolution module. 
Predicted joints should behave like real joints for real articulated part transformations and part-level SE(3) equivariant features learning.
% such that 1) parts in the canonical object space are more likely to transform like real articulated parts; 2) the designed pose-aware point convolution module can output better part-level equivariant features. 
% should behave like real ones for the following two reasons: 
% 1) the part kinematic constraints can then be added more correctly; 
% % such that part kinematic constraints can be added more correctly, 
% 2) estimated part poses can better facilitate the pose-aware point convolution module calculate part-level equivariant features. 
% \subsummary{Purpose}
% the part-level equivariant feature extraction
% Besides, to make the predicted joints behave like a real joint, 
% joint direction and pivot point behave like a joint, 
% we add constraints between such predicted joint parameters and reconstructed shapes of such two adjacent parts.
% the shape reconstruction of such two adjacent parts. 
% In the method, we regress the joint direction and pivot point from corresponding part or part-pair features, which are further used to calculate rotation matrix and translation vector for the part in the shape canonical space. 
% todo: need to quote previous strategy for joint prediction?
% Such a regression based method is different from the bottom-up joint prediction strategy which regresses point offsets from the joint and calculates joint direction and location using the predicted offsets of points near to the joint~\cite{li2020category}. 
% The reason to adopt a regression based strategy is the heavy supervision needed for dense offset regression that is not that friendly for the unsupervised setting. 
% However, just treating the predicted joint axis direction as the rotation axis direction is not sufficient for predicting real joints. 
However, just predicting joint parameters for computing rotation matrices is not sufficient to predict real joints. 
% \subsummary{Necessity}
% Therefore, we propose a point-based joint regularization term based on the assumption that the joint between two parts $i,j$ should go through the two adjacent part shapes connected by it both before and after the articulation transformation in the canonical space. 
% To predict the joint $\{ \mathbf{u}_{i,j}, \mathbf{p}_{i,j}^v \}$ between two adjacent parts $\hat{\mathbb{S}}_i, \hat{\mathbb{S}}_j$ for part transformation in the shape canonical space, some constraints are needed to be added to the predicted axis direction and pivot point to make the predicted joint a reasonable one. 
% The constraint is added based on the assumption that the joint between two parts $i,j$
% part joint 
% should go through the two adjacent part shapes connected by it both before and after the articulation transformation in the canonical space.
% after and before part articulation transformation. 
%  in the shape canonical space before and after part rigid transformation ($\mathbf{P}_i^{SC}, \mathbf{P}_j^{SC}, \mathbf{P}_i^{PC} + \mathbf{p}_i^c, \mathbf{P}_j^{PC} + \mathbf{p}_j^c$) connected by it. 
% A popular strategy adopted by previous works is regressing points' offset to the joint and using coordinates of points near to the joint to calculate the joint's aixs direction and location~\cite{li2020category}. 
% This method requires dense supervision and is not friendly to be transferred to an unsupervised setting directly. 
% Thus, we choose to predict the joint axis direction and pivot point directly from the obtained part equivariant features. And add some constraints for the predicted part axises and pivot points based on part shapes and joint parameters. 
% To add such constraint, we make an assumption on the joint $\{ \mathbf{u}_i, \mathbf{q}_i\}$ and part shapes reconstruction $\hat{\mathbb{S}}_i, \hat{\mathbb{S}}_j$: the joint $\mathbf{u}_i$ must be adjacent to two reconstructed part shapes $\hat{\mathbb{S}}_i$ and $\hat{\mathbb{S}}_j$. 
% Based on the assumption, 
Therefore, we devise a point-based joint constraint term
% for predicted joints 
% add constraints on the predicted joint 
for each predicted joint $(\mathbf{u}_i^{g_0}, \mathbf{p}_{i,j}^v)$, 
% $\{(\mathbf{u}_i^{g_0}, \mathbf{p}_{i,j}^v)\}$, 
where $g_0 = \text{argmin}_{g\in G}d(X, Y^g)$ (Eq.~\ref{eq_recon_loss}).
% is the index of the selected reconstruction hypothesis that achieves the minimum distance value $d(X, Y^{g_0})$. 
% \subsummary{Method overview}
%%%% move to supp %%%%
% It is based on the assumption that the joint between two parts $i,j$ should go through the two adjacent part shapes connected by it both before and after the articulation transformation in the canonical space. 
%%%% move to supp %%%%
% \subsummary{Assumption}
Specifically, given the predicted pivot point $\mathbf{p}_{i,j}^v$ and joint direction $\mathbf{u}_i^{g_0}$, we independently randomly sample a set of points from the joint by shifting the pivot point $\mathbf{p}_{i,j}^v$: $P_{i,j}^v = \{ \mathbf{p}_{i,j}^{v,k} \vert 0\le k\le K^v\}$. 
%%%%%%%%%%%%%%%
% offset scales from a uniform distribution: $\{ s_k \vert s_k \sim \mathcal{U}(a,b), 1\le k\le K^v \}$, where $ a\in \mathbb{R} < b \in \mathbb{R}$ are hyper-parameters that can be tuned for each category. 
% After that, a set of shifted pivot points are generated via $\{ \mathbf{p}_{i,j}^{v,k} = \mathbf{p}_{i,j}^v + s_k \cdot \mathbf{u}_i^{g_0} \vert 1\le k\le K^v \}$, where $K^v$ is the number of sampled shifted pivot points. 
% Together with the pivot point, also denoted as $\mathbf{p}_{i,j}^{v,0}$, we get the (shifted) pivot point set $P_{i,j}^v = \{ \mathbf{p}_{i,j}^{v,k} \vert 0\le k\le K^v\}$.
%%%%%%%%%%%%%%%
% where $K^v$ is the number of sampled shifted pivot points. 
% Loss for joint constraints are added as follows:
The joint regularization loss term is as follows: 
% Denote shapes of part $i$ in the canonical object space before and after the articulated transformation as $Z_i^1$ and $Z_i^2$ respectively,
% % Assume shapes of part $i$ in the canonical object space before and after the articulated transformation are denoted as $Z_i^1$ and $Z_i^2$ respectively, 
% the loss for joint regularization is designed as follows: 
\begin{align*}
    \mathcal{L}_{reg} = \sum_{(i,j)\in \mathcal{E}_{\mathcal{T}}} d(P_{i,j}^v, Z_i^2) + d(P_{i,j}^v, Z_j^2) + d(P_{i,j}^v, Z_i^1) + d(P_{i,j}^v, Z_j^1),
\end{align*}
% \begin{align*}
%     \mathcal{L}_{reg} = \sum_{(i,j)\in \mathcal{E}_{\mathcal{T}}} d(P_{i,j}^v, \mathbf{R}_i^{g_0,o} Z_i' + \mathbf{t}_i^{g_0,o}) + d(P_{i,j}^v, \mathbf{R}_j^{g_0,o} Z_j' + \mathbf{t}_j^{g_0,o}) + d(P_{i,j}^v, Z_i') + d(P_{i,j}^v, Z_j'),
% \end{align*}
where $Z_i^1$ and $Z_i^2$ are shapes of part $i$ in the canonical object space before and after its articulated, 
$\mathcal{E}_{\mathcal{T}}$ is the set of adjacent parts,  $d(X_1, X_2)$ is the unidirectional Chamfer Distance function from point cloud $X_1$ to $X_2$.
% \subsummary{Approach}
% $j_0$ is the index of the selected pose hypothesis that achieves the minimum distance value $d(X, Y^{j_0})$. 
Therefore, our self-supervised shape reconstruction loss is a linear combination of the above two loss terms: 
% Thus, the total loss for the self-supervised shape reconstruction task is 
$\mathcal{L} = \mathcal{L}_{rec} + \lambda \mathcal{L}_{reg}$, where $\lambda$ is a hyper-parameter. 
% \subsummary{Summary for loss}

% \zz{??}

%%% move to supp? %%%%
% \vpara{Iterative Pose Estimation.}
% It can be noticed that the designed part-level equivariant network needs estimated per-point pose as input. 
% The ideal part-level equivariance can only be achieved when the input per-point pose is accurate. 
% Therefore, we design an iterative pose estimation approach where the estimated pose from the previous iteration is taken as the input per-point pose in the current iteration. 
% We wish that the pose estimation quality can be improved across such iterations. 



==> articles/repro_state.tex <==
\section{Reproducibility Statement}

\vpara{Novel Models and Algorithms.}
Our method is composed of two novel designs: 
1) Part-level SE(3) equivariant network; 
2) Part Shape, Structure, Pose Disentanglement Strategy. 
Please refer to \emph{Key Implementations} section in the file \emph{equi-articulated-pose/README.md} in our Supplementary Materials. 
For each key design/component, we provide the implementation reference to our submitted code in the file. 

\vpara{Theoretical Results.}
Please refer to section~\ref{sec_appen_part_level_equiv} in the Appendix for the proof of the part-level SE(3) equivariant property of our pose-aware point convolution strategy. 

\vpara{Experiments.} 
For experiments, we provide 1) Source code.
% of our implementation. 
Please refer to the folder \emph{equi-articulated-pose} in our Supplementary Materials for details. 2) Details of the data preparation process. Please refer to the section~\ref{sec_appen_data_prepare} in the Appendix for details. 3) Implementation details of our method and compared baselines. Please refer to the section~\ref{sec_appen_imple_details} and~\ref{sec_appen_baselines} in the Appendix. 
4) Category-level articulated object pose evaluation strategy. 
Please refer to the section~\ref{sec_appen_eval} for details. 
We also provide related references to the code in the \emph{README.md} file. 
